Obfuscation of Pseudo-Deterministic Quantum Circuits

We show how to obfuscate pseudo-deterministic quantum circuits in the classical oracle model, assuming the quantum hardness of learning with errors. Given the classical description of a quantum circuit $Q$, our obfuscator outputs a quantum state $\ket{\widetilde{Q}}$ that can be used to evaluate $Q$ repeatedly on arbitrary inputs. Instantiating the classical oracle using any candidate post-quantum indistinguishability obfuscator gives us the first candidate construction of indistinguishability obfuscation for all polynomial-size pseudo-deterministic quantum circuits. In particular, our scheme is the first candidate obfuscator for a class of circuits that is powerful enough to implement Shor's algorithm (SICOMP 1997). Our approach follows Bartusek and Malavolta (ITCS 2022), who obfuscate \emph{null} quantum circuits by obfuscating the verifier of an appropriate classical verification of quantum computation (CVQC) scheme. We go beyond null circuits by constructing a publicly-verifiable CVQC scheme for quantum \emph{partitioning} circuits, which can be used to verify the evaluation procedure of Mahadev's quantum fully-homomorphic encryption scheme (FOCS 2018). We achieve this by upgrading the one-time secure scheme of Bartusek (TCC 2021) to a fully reusable scheme, via a publicly-decodable \emph{Pauli functional commitment}, which we formally define and construct in this work. This commitment scheme, which satisfies a notion of binding against committers that can access the receiver's standard and Hadamard basis decoding functionalities, is constructed by building on techniques of Amos, Georgiou, Kiayias, and Zhandry (STOC 2020) introduced in the context of equivocal but collision-resistant hash functions.

==> Construction.tex <==
% !TEX root = main.tex
\section{Obfuscation}

\subsection{Construction}

Also, let $U[x]$ be the universal quantum circuit with an input $x$ hard-coded. That is, $U[x]$ takes as input the description of a circuit $Q$ and outputs $Q(x)$.

The obfuscation procedure is given in \proref{fig:QObf} and the evaluation procedure on input $x$ is given in \proref{fig:QEval}. This evaluation procedure includes measurements as written, so it may not be clear that the obfuscation is reusable. However, we will show that correctness holds with $1-\negl(\secp)$, which implies that the evaluator could run coherently, measure the output bit $b$, and then reverse their computation, allowing them to evaluate the circuit on an arbitrary (polynomial) number of inputs of their choice.



\protocol{$\underline{\Eval(\widetilde{Q},x)}$}{Protocol for evaluating an obfuscation of pseudo-deterministic quantum circuit $Q$ on input $x$.}{fig:QEval}{
\begin{itemize}
    \item Parse $\widetilde{Q}$ as $\left(\ct,\ket{\sk},\ket{\ck},\cO(P_\Com),\cO(P_\Gen),\cO(P_\Out)\right)$, and $\ket{\ck}$ as $\{\ket{\ck_{i,j}}\}_{i \in [r], j \in [\ell]}$.
    \item Prepare $\ket{\psi_{\ct,U[x]}}^{\sB_1},\dots,\ket{\psi_{\ct,U[x]}}^{\sB_r} \gets \cP_\Prep^\CV(\ct,U[x])$.
    
    
   %Given $(\ct,U[x])$, prepare $r$ copies of the state \[\ket{\psi_{\ct,U[x]}} \coloneqq \sum_{m \in \{0,1\}^\ell}\alpha_m\ket{m}^{\sM_i},\] as done by $\cP^\CV$.
    \item For each $i \in [r], j \in [\ell]$ apply $\PO.\Com^{\PO.\OZ[\dk_{i,j}],\PO.\OX[\dk_{i,j}]}$ to register $\sB_{i,j}$ and $\ket{\ck_{i,j}}$ to produce an output on register $(\sB_{i,j},\sS_{i,j})$. This operation requires using $\ket{\sk}$ to sign $0^{n+1}$, and then querying $\cO(P_\Com)$ to obtain access to the oracles $\PO.\OZ[\dk_{i,j}]$ and  $\PO.\OX[\dk_{i,j}]$.
    
    %Using the states $\ket{\sk},\ket{\ck}$ and oracle $\cO(P_\Com)$, apply 
    
    
    %prepare the state \[\ket{\psi_{\ct,U[x]}'}^{\sM_i,\sV_{i,1},\dots,\sV_{i,\ell}} \coloneqq \sum_{m \in \{0,1\}^\ell}\alpha_m\ket{m}^{\sM_i}\ket{\bS_{i,1}^{m_1}}^{\sV_{i,1}}\dots\ket{\bS_{i,\ell}^{m_\ell}}^{\sV_{i,\ell}}\] for each $i \in [r]$.
    \item Compute $\Tok.\Sign((1,x),\ket{\sk})$ to obtain $\sigma_x$.
    \item Query $\cO(P_\Gen)$ on $(x,\sigma_x)$ to obtain $\pp_{x,\sigma_x}$.
    \item Apply $\cP^\CV_\Prove(\sB_1,\dots,\sB_r,\pp_{x,\sigma_x})$ to obtain classical strings $\{y_{i,j},z_{i,j}\}_{i \in [r], j \in [\ell]}$. Let $T \coloneqq H(y_{1,1},\dots,y_{r,\ell})$
    \item For each $i: T_i = 0, j \in [\ell]$, apply $\OpenZ$ to registers $(\sB_{i,j},\sS_{i,j})$ to obtain classical string $v_{i,j}$.
    \item For each $i: T_i = 1, j \in [\ell]$, apply $\OpenX$ to registers $(\sB_{i,j},\sS_{i,j})$ to obtain classical string $v_{i,j}$.
    \item Query $\cO(P_\Out)$ on $(x,\sigma_x,\{y_{i,j},v_{i,j},z_{i,j}\}_{i \in [r], j \in [\ell]})$ to obtain $b$, and output $b$.
\end{itemize}

}

\subsection{Security proof}

\begin{theorem}
The scheme $(\Obf,\Eval)$ described in \proref{fig:QObf} and \proref{fig:QEval} is a VBB obfuscator for pseudo-deterministic quantum circuits (\cref{def:ideal-obfuscation}).
\end{theorem}

\begin{proof}
First, for any adversary $\cA = \cA_\secp$ we describe a simulator $\cS = \cS_\secp$.
\begin{itemize}
    \item Sample $\ct \gets \Enc(\pk_\QFHE,0)$, $(\vk,\ket{\sk}) \gets \Tok.\Gen(1^\secp,n+1)$, and $\{(\dk_{i,j},\ket{\ck_{i,j}}) \gets \PO.\Gen(1^\secp)\}_{i \in [r], j \in [\ell]}$. Let $\ket{\ck} = (\ket{\ck_{1,1}},\dots,\ket{\ck_{r,\ell}})$. 
    \item Let $\cB$ be the classical VBB obfuscation simulator, defined based on $\cA$.%guaranteed to exist by the VBB obfuscator $\cO$ for classical circuits.
    \item Initialize $\cB$ with $(\ct,\ket{\sk},\ket{\ck})$. Whenever $\cB$ makes a query to its oracle implementing $P_\Com,P_\Gen$, or $P_\Out$, answer honestly except for the following difference. For each query $(x,\sigma_x,\pi)$ to $P_\Out$, in the case that the output of $\cV_\Ver^\CV$ is not $\bot$, then query the oracle $O[Q]$ on input $x$ to receive $b$, and output $b$.
\end{itemize}
Now, we describe a sequence of hybrids, each of which outputs a single bit.
\begin{itemize}
    \item $\cH_0$: This is the output of $\cA$ upon receiving $\widetilde{Q}$.
    \item $\cH_1$: This is the output of $\cB^{P_\Com,P_\Gen,P_\Out}(\ct,\ket{\sk},\ket{\ck})$.
    \item $\cH_2$: Same as $\cH_1$, except that queries to $P_\Out$ are answered as in the description of the simulator above.
    \item $\cH_3$: Same as $\cH_2$, except that $\ct$ is sampled as an encryption of 0. This describes the simulator $\cS$.
\end{itemize}
Note that \[|\Pr[\cH_0 = 1] - \Pr[\cH_1 = 1]| = \negl(\secp)\] follows immediately from the security of $\cO$, and \[|\Pr[\cH_2 = 1] - \Pr[\cH_3 = 1]| = \negl(\secp)\] follows immediately from the security of QFHE, since $\sk_\QFHE$ is not used in $\cH_2$. Therefore, it suffices to show that $\cH_1$ and $\cH_2$ are indistinguishable, which is shown in the following lemma.

\end{proof}

\begin{lemma}
$|\Pr[\cH_1 = 1] - \Pr[\cH_2 = 1]| = \negl(\secp).$
\end{lemma}

\begin{proof}
Suppose that the lemma is false. Then there must exist some $(\pk_\QFHE,\sk_\QFHE) \in \QFHE.\Gen(1^\secp), \ct \gets \Enc(\pk_\QFHE,Q)$ and an index $p$ such that, when $\cB$ is initialized with $\ct$, $\cB$'s $p$'th query to its oracle implementing $P_\Out$ has non-negligible amplitude on strings $(x,\sigma_x,\pi)$ such that $P_\Out(x,\sigma_x,\pi) = 1 - Q(x)$.

Now, we define an oracle algorithm $\cC^G$ that has $(\pk_\QFHE,\sk_\QFHE,\ct)$ hard-coded and operates as follows.

\begin{itemize}
    \item Sample $(\vk,\ket{\sk}) \gets \Tok.\Gen(1^\secp,n+1)$, and $\{(\dk_{i,j},\ket{\ck_{i,j}}) \gets \PO.\Gen(1^\secp)\}_{i \in [r], j \in [\ell]}$. Let $\ket{\ck} = (\ket{\ck_{1,1}},\dots,\ket{\ck_{r,\ell}})$.
    \item Run $\cB^{P_\Com,P_\Gen,P_\Out}(\ct,\ket{\sk},\ket{\ck})$ until right before its $p$'th query to $P_\Out$. Answer all of $\cB$'s oracle queries internally, except that whenever the random oracle $G$ is invoked (during a call to $P_\Gen$ or $P_\Out$), forward this query an external random oracle $G$. 
    \item Measure part of the query register in the computational basis to obtain classical string $(x,\sigma_x)$.
    \item Let $\sP$ be the register holding the remainder of the query register, which contains a superposition over proofs $\pi$, let $\sB$ be the remainder of $\cB$'s state, and let $\sR$ be a register that holds the classical information $(\pk_\QFHE,\sk_\QFHE,\ct,\vk,\{\dk_{i,j}\}_{i,j})$ sampled at the beginning. Output classical string $(x,\sigma)$ and a left-over quantum state on register $\sV = (\sP,\sB,\sR)$.
\end{itemize}

Note that $\cC$ makes $q = \poly(\secp)$ total queries to $G$, since $\cB$ is QPT. 

Next, we define a family of projections $\{\Pi_{(x,\sigma_x),r}\}_{(x,\sigma_x),r}$ on register $\sV$, where $\Pi_{(x,\sigma),r}$ projects onto $\pi$ (on register $\sP$) such that $P_\Out^{r,\sR}(x,\sigma,\pi) = 1-Q(x)$. $P_\Out^{r,\sR}$ is the procedure $P_\Out$ where $r$ is used to generate $(\pp_{x,\sigma_x},\sparam_{x,\sigma_x}) \coloneqq \cV_\Gen^\CV(\ct,U[x];r)$, and the classical information $\pk_\QFHE, \sk_\QFHE, \ct,\vk,\{\dk_{i,j}\}_{i,j}$ that is used during the procedure comes from register $\sR$.

Thus, we have that \[\E\left[\Tr\left(\Pi_{(x,\sigma_x),G(x,\sigma_x)}(\tau)\right) : ((x,\sigma_x),\tau) \gets \cC^G\right] = 1/\poly(\secp),\]

and by \cref{thm:measure-and-reprogram}, since $q = \poly(\secp)$, there exists $\Sim^\cC$ such that

\[\E\left[\Tr\left(\Pi_{(x,\sigma_x),r}(\tau)\right) : \begin{array}{r} ((x,\sigma_x),\rho) \gets \Sim^\cC \\ r \gets \{0,1\}^\secp \\ \tau \gets \Sim^\cC(r,\rho)\end{array}\right] = 1/\poly(\secp).\]

Next, we define $\widetilde{\Sim}^\cC$ to be the same as $\Sim^\cC$, except that in the second stage, each query made by $\cB$ to $P_\Com$ is answered with $\bot$. 

\begin{claim}
\[\E\left[\Tr\left(\Pi_{(x,\sigma_x),r}(\tau)\right) : \begin{array}{r} ((x,\sigma_x),\rho) \gets \widetilde{\Sim}^\cC \\ r \gets \{0,1\}^\secp \\ \tau \gets \widetilde{\Sim}^\cC(r,\rho)\end{array}\right] = 1/\poly(\secp).\]
\end{claim}

\begin{proof}
We can condition on $\Tok.\Ver(\vk,(1,x),\sigma_x) = \top$, since this is checked as a part of $\Pi_{(x,\sigma_x),r}$. Then, by the 1-strong-unforgeability of $\Tok$ (\cref{def:unforgeability}), once $(x,\sigma_x)$ is output, $\cB$ cannot produce any signature $\sigma'$ such that $\Tok.\Ver(\vk,0^{k+1},\sigma') = \top$ except with negligible probability, which completes the proof.
\end{proof}

Next, we define $\widetilde{\Pi}_{(x,\sigma_x),r}$ to be the same as $\Pi_{(x,\sigma_x),r}$ except that any $\pi$ such that $\mathsf{TestRoundOutputs}[\sparam_{x,\sigma_x}](\pi) \notin D_\out[\sk_\QFHE,Q(x)]$ is rejected. 

\begin{claim}
\[\E\left[\Tr\left(\widetilde{\Pi}_{(x,\sigma_x),r}(\tau)\right) : \begin{array}{r} ((x,\sigma_x),\rho) \gets \widetilde{\Sim}^\cC \\ r \gets \{0,1\}^\secp \\ \tau \gets \widetilde{\Sim}^\cC(r,\rho)\end{array}\right] = 1/\poly(\secp).\]
\end{claim}

\begin{proof}
This follows directly from \cref{lemma:Q-out}.
\end{proof}

Finally, we will define a sequence of hybrids $\{\cH_h\}_{h \in [0,q]}$ based on $\widetilde{\Sim}^\cC$. The value of each hybrid, denoted $\E[\cH_h]$ is defined to be $\E[\Tr(\widetilde{\Pi}_{(x,\sigma_x),r}(\tau))]$, but we will change how $\tau$ is sampled in each hybrid. Hybrid $\cH_h$ is defined as follows.

\begin{itemize}
    \item Recall from \cref{thm:measure-and-reprogram} that the first part of $\widetilde{\Sim}^\cC$ answers $\cC$'s oracle queries with $G$ honestly, and that at some point (determined by $(i,b)$) the second part of $\widetilde{\Sim}^\cC$ starts answering $\cC$'s oracle queries with $G[(x,\sigma_x) \to r]$. 
    \item Run $((x,\sigma_x),\rho) \gets \widetilde{\Sim}^\cC$ and sample $r \gets \{0,1\}^\secp$.
    \item Run $\tau \gets \widetilde{\Sim}^\cC(r,\rho)$ with the following difference. For the first $h$ times that $\cB$ queries $P_\Out$ after $\widetilde{\Sim}^\cC$ has started using the oracle $G[(x,\sigma_x) \to r]$, answer the $P_\Out$ query with $\bot$.
\end{itemize}

Note that $\cH_0$ is just $\widetilde{\Sim}^\cC$ described above. Since $q = \poly(\secp)$, we see that a combination of the following two claims would give us a contradiction, completing the proof.

\begin{enumerate}
    \item For any $h \in [q]$, $\E[\cH_h] \geq \E[\cH_{h-1}] - \negl(\secp)$.
    \item $\E[\cH_q] = \negl(\secp)$.
\end{enumerate}

%\begin{lemma}\label{lemma:final-hybrid}
%$\E[\cH_q] = \negl(\secp)$.
%\end{lemma}

The proof of the second claim follows directly from the soundness of $\Pi^\CV$ (\cref{lemma:soundness}), since $\widetilde{\Sim}^\cC$ only needs $\pp_{x,\sigma_x}$ (and not $\sparam_{x,\sigma_x}$) to obtain $\tau$, where $(\pp_{x,\sigma_x},\sparam_{x,\sigma_x}) \coloneqq \cV_\Gen^\CV(\ct,U[x];r)$. Thus, $\widetilde{\Sim}^\cC$ (with oracle access to the random oracle $H$) can be seen as an adversarial prover for $\Pi^\CV$. 
Thus, to complete the proof, it suffices to prove the first claim, which is stated as a lemma below.

%has non-negligible amplitude on $(x,\sigma_x,\pi)$ such that (1) $\sigma_x$ is a valid signature on $x$, (2) $\cV_\Ver^\CV$ accepts $\pi$, and (3) $\cV_\Out^\CV$ outputs $1-Q(x)$. In what follows, we show that this would violate the security of either $\Pi^\CV, \Tok,$ or $\PO$.

\end{proof}

\begin{lemma}\label{lemma:intermediate-hybrids}
For any $h \in [q]$, $\E[\cH_h] \geq \E[\cH_{h-1}] - \negl(\secp)$.
\end{lemma}

\begin{proof}

We prove this by consider a sequence of sub-hybrids. In $\cH_{h-1}$, let $h^*$ denote the first query that $\cB$ makes to $P_\Out$ in the second stage of $\Sim^\cC$ such that $P_\Out$ is not instructed to always output $\bot$. So, if the hybrid were $\cH_h$, this query would be always answered with $\bot$.

\begin{itemize}
    \item $\cH_{h-1,0}$ is $\cH_{h-1}$.
    \item $\cH_{h-1,1}$ is the same as $\cH_{h-1,0}$, except that query $h^*$ answers any $(x',\sigma'_{x'},\pi')$ such that $(x',\sigma'_{x'}) \neq (x,\sigma_x)$ with $\bot$.
    \item $\cH_{h-1,2}$ is the same as $\cH_{h-1,1}$, except that query $h^*$ answers any $(x,\sigma_x,\pi)$ such that $\mathsf{TestRoundOutputs}[\sparam_{x,\sigma_x}](\pi) \notin D_\mathsf{in}[\sk_\QFHE,Q(x)]$ with $\bot$.
    \item $\cH_{h-1,3}$ is the same as $\cH_{h-1,2}$, except that query $h^*$ is always answered with $\bot$. This is equivalent to $\cH_{h}$.
. 
\end{itemize}

Now, we show that following sequence of claims.

\begin{claim}
$\E[\cH_{h-1,1}] \geq \E[\cH_{h-1,0}] - \negl(\secp)$.
\end{claim}

\begin{proof}
This follows from the 1-strong-unforgeability of $\Tok$ (\cref{def:unforgeability}). Indeed, $(x,\sigma_x)$ has previously been output, and we can condition on $\Tok.\Ver(\vk,(1,x),\sigma_x) = \top$, since this is checked as part of $\Pi_{(x,\sigma_x),r}$. Thus, obtaining any $(x',\sigma'_{x'}) \neq (x,\sigma_x)$ such that $\Tok.\Ver(\vk,(1,x'),\sigma'_{x'})$ with noticeable probability would violate \cref{def:unforgeability}.
\end{proof}

\begin{claim}
$\E[\cH_{h-1,2}] \geq \E[\cH_{h-1,1}] - \negl(\secp)$.
\end{claim}

\begin{proof}
This follows directly from \cref{lemma:Q-in}.
\end{proof}

\begin{claim}
$\E[\cH_{h-1,3}] \geq \E[\cH_{h-1,2}] - \negl(\secp)$.
\end{claim}

\begin{proof}

Let $m \coloneqq |W|$, where $W$ is defined in \cref{subsec:2-message}, to be the indices that contain the output ciphertexts for some given $(\pp,\sparam)$. We note that $m = |W|$ is the same for all $(\pp,\sparam) \in \Gen(1^\secp)$ for some fixed security parameter $\secp$, circuit $U[x]$ and ciphertext $\ct$ encrypting $Q$.

Now we define an oracle algorithm $\cD$ as follows.

\begin{itemize}
    \item $\cD$ takes as input $\{\ket{\ck_\iota}\}_{\iota \in [m]}$, where $\{\dk_\iota, \ket{\ck_\iota} \gets \PO.\Gen(1^\secp)\}_{\iota \in [m]}$.
    \item $\cD$ samples $r \gets \{0,1\}$ and sets $(\pp,\sparam) \coloneqq \cV^\CV_\Gen(\ct,U[x];r)$. Let $W$ be the subset of indices $i \in [r], j \in [\ell]$ defined in \cref{subsec:2-message}. For $(i,j) \notin W$, sample $\dk_{i,j},\ket{\ck_{i,j}} \gets \PO.\Gen(1^\secp)$, and re-define $\{\ket{\ck_\iota}\}_{\iota \in [m]}$ as $\{\ket{\ck_{i,j}}\}_{(i,j) \in W}$.
    \item $\cD$ runs $\widetilde{\Sim}^\cC$ as defined by $\cH_{h-1,2}$ until right before query $h^*$ is answered. Any queries to $\PO.\OZ[\dk_{i,j}]$ or $\PO.\OX[\dk_{i,j}]$ for $(i,j) \in W$ are forwarded to external oracles with $\{\dk_{i,j}\}_{(i,j) \in W}$ hard-coded. 
\end{itemize}

That is, we can write the operation of $\cD$ as

\[\ket{\psi} \gets \cD^{\PO.\OZ[\dk],\PO.\OX[\dk]}(\ket{\ck}),\] where $\{\dk_\iota, \ket{\ck_\iota} \gets \PO.\Gen(1^\secp)\}_{\iota \in [m]}$, $\ket{\ck} = (\ket{\ck_1},\dots,\ket{\ck_m})$, $\OZ[\dk]$ is the collection of oracles $\OZ[\dk_1],\allowbreak\dots,\allowbreak\OZ[\dk_m]$, and $\OX[\dk]$ is the collection of oracles $\OX[\dk_1],\dots,\OX[\dk_m]$.

We name two registers of $\ket{\psi}$ as follows. 

\begin{itemize}
    \item Register $\sS$ contains the current state of $\widetilde{\Sim}^\cC$, including the $h^*$ query register.
    \item Register $\sA$ contains a classical string consisting of all the classical information that has been hard-coded, sampled, or measured by $\cD$: $(x,\sigma_x,r,Q,\pk_\QFHE,\sk_\QFHE,\ct,\vk,\{\dk_{i,j}\}_{(i,j) \notin W},s)$, where $s$ is any information sampled by $\widetilde{\Sim}$.
\end{itemize}
 
Next, we define an oracle unitary $\cU[2]$ as follows.

\begin{itemize}
    \item $\cU[2]$ takes as input the state $\ket{\psi}$ output by $\cD$.
    \item It coherently runs the remainder of $\widetilde{\Sim}^\cC$ as defined by $\cH_{h-1,2}$. Any queries to $\PO.\OZ[\dk_{i,j}]$ for $(i,j) \in W$ are forwarded to external oracles. Note that this portion of $\widetilde{\Sim}^\cC$ does not requires access to oracles $\PO.\OX[\dk_{i,j}]$ for $(i,j) \in W$.
\end{itemize}

That is, we can write the operation of $\cU[2]$ as 

\[\ket{\psi'} \coloneqq \cU[2]^{\PO.\OZ[\dk]}(\ket{\psi}).\]

We also define $\cU[3]$ to be identical to $\cU[2]$ except that it runs the remainder of $\widetilde{\Sim}^\cC$ as defined by $\cH_{h-1,3}$. Note that the only difference between $\cU[2]$ and $\cU[3]$ is how the $h^*$ query answered.

Next, we define two projectors. 

\begin{itemize}
    \item $\Pi_{h^*}$ projects onto $(x,\sigma_x,\pi)$ on the $h^*$ query register (part of $\sS$) such that $P_\Out(x,\sigma_x,\pi) \neq \bot$ in $\cH_{h-1,2}$. The classical information defining $P_\Out$ is obtained from register $\sA$.
    \item $\Pi_{\mathsf{final}}$ applies $\widetilde{\Pi}_{x,\sigma,r}$, where the classical information defining this projector is obtained from register $\sA$.
\end{itemize}

For any state $\ket{\psi}$ output by $\cD$, we write $\ket{\psi} \coloneqq \ket{\psi_\top} + \ket{\psi_\bot}$, where $\ket{\psi_\top} \coloneqq \Pi_{h^*}\ket{\psi}$. Next, we notice that for any such $\ket{\psi_\bot}$, $\cU[2]\ket{\psi_\bot} = \cU[3]\ket{\psi_\bot}$, since they both always answer the $h^*$ query with $\bot$.

Now, observe that \[\E[\cH_{h-1,2}] = \E_{\dk,\ket{\ck}}\left[\bigg\| \Pi_{\mathsf{final}}\cU[2]^{\PO.\OZ[\dk]}(\ket{\psi_\top} + \ket{\psi_\bot})\bigg\|^2 : \ket{\psi_\top} + \ket{\psi_\bot} \gets \cD^{\PO.\OZ[\dk],\PO.\OX[\dk]}(\ket{\ck})\right],\] and \[\E[\cH_{h-1,3}] = \E_{\dk,\ket{\ck}}\left[\bigg\| \Pi_{\mathsf{final}}\cU[3]^{\PO.\OZ[\dk]}(\ket{\psi_\top} + \ket{\psi_\bot})\bigg\|^2 : \ket{\psi_\top} + \ket{\psi_\bot} \gets \cD^{\PO.\OZ[\dk],\PO.\OX[\dk]}(\ket{\ck})\right],\] so by the above observation,

\[\E[\cH_{h-1,2}] - \E[\cH_{h-1,3}] \leq \E_{\dk,\ket{\ck}}\left[3\bigg\| \Pi_{\mathsf{final}}\cU[2]^{\PO.\OZ[\dk]}\ket{\psi_\top}\bigg\| : \ket{\psi_\top} + \ket{\psi_\bot} \gets \cD^{\PO.\OZ[\dk],\PO.\OX[\dk]}(\ket{\ck})\right],\] and thus it suffices to show that 

\[\E_{\dk,\ket{\ck}}\left[\bigg\| \Pi_{\mathsf{final}}\cU[2]^{\PO.\OZ[\dk]}\Pi_{h^*}\ket{\psi}\bigg\|^2 : \ket{\psi} \gets \cD^{\PO.\OZ[\dk],\PO.\OX[\dk]}(\ket{\ck})\right] = \negl(\secp).\]

Now, suppose that $\cD$ is re-defined to permute its registers so that the first registers it outputs are the parts of the proof $\pi$ that is on indices in $W$. We then define $\Pi_{\dk,\mathsf{in}}$ to be the projector that reads $(Q,x,\sk_\QFHE)$ and applies $\Pi_{\dk,D_{\mathsf{in}}[\sk_\QFHE,Q(x)]}$ to these registers and define $\Pi_{\dk,\out}$ to be the projector that reads $(Q,x,\sk_\QFHE)$ and applies $\Pi_{\dk,D_\out[\sk_\QFHE,Q(x)]}$ to these registers. Then, by the definition of $\Pi_{h^*}$ and $\Pi_{\mathsf{final}}$, it holds that the above expectation is bounded by

\[\E_{\dk,\ket{\ck}}\left[\bigg\|\Pi_{\dk,\out} \cU[2]^{\PO.\OZ[\dk]} \Pi_{\dk,\mathsf{in}}\ket{\psi}\bigg\|^2 : \ket{\psi} \gets \cD^{\PO.\OZ[\dk],\PO.\OX[\dk]}(\ket{\ck})\right].\]

Since $\sk_\QFHE$ has been fixed, we can define $\Pi_{\dk,\mathsf{in},0} \coloneqq \Pi_{\dk,D_{\mathsf{in}}[\sk_\QFHE,0]}$ and $\Pi_{\dk,\mathsf{in},1} \coloneqq \Pi_{\dk,D_{\mathsf{in}}[\sk_\QFHE,1]}$, and note that the above expectation can be bounded by 

\[\sum_{b \in \{0,1\}}\E_{\dk,\ket{\ck}}\left[\bigg\|\Pi_{\dk,\out,b} \cU[2]^{\PO.\OZ[\dk]} \Pi_{\dk,\mathsf{in},b}\ket{\psi}\bigg\|^2 : \ket{\psi} \gets \cD^{\PO.\OZ[\dk],\PO.\OX[\dk]}(\ket{\ck})\right].\]

Finally, by the $m$-predicate-binding of $\PO$, we know that for each fixed $b \in \{0,1\}$, 

\[\E_{\dk,\ket{\ck}}\left[\bigg\|\Pi_{\dk,\out,b} \cU[2]^{\PO.\OZ[\dk]} \Pi_{\dk,\mathsf{in},b}\ket{\psi}\bigg\|^2 : \ket{\psi} \gets \cD^{\PO.\OZ[\dk],\PO.\OX[\dk]}(\ket{\ck})\right] = \negl(\secp),\] which completes the proof.



%This follows from the $|D|$-predicate-binding (\cref{def:predicate-binding}) of $\PO$, where $D$ is the domain of $\mathsf{OutPattern}$. Consider the state $\ket{\psi}$ of $\cH_{h-1,2}$ right before $h^*$ is answered. The component of $\ket{\psi}$ that is accepted by $P_\Out$ contains $\PO$ openings to strings in $P_{\mathsf{in},Q(x)}$, while the component that is eventually accepted by $\widetilde{\Pi}_{x,\sigma_x}$ contains $\PO$ openings to strings in $P_{\out,Q(x)}$. Since $P_{\mathsf{in},Q(x)}$ and $P_{\out,Q(x)}$ are incompatible predicates, these components must have negligible overlap, by the $|D|$-predicate-binding of $\PO$. Thus, altering the component that is accepted by $P_\Out$ will only negligibly affect the component that is eventually accepted by $\widetilde{\Pi}_{x,\sigma_x}$, completing the proof. \james{TODO: make reduction and analysis more formal}
\end{proof}


\end{proof}



==> QFHE-verification.tex <==
% !TEX root = main.tex
\section{Verification of QFHE evaluation}\label{sec:CVQC}

\iffalse
\subsection{$\text{QPIP}_1$ verification}

Let $(\Gen,\Enc,\Eval,\Dec)$ be a quantum fully-homomorphic encryption (QFHE) scheme. In \cref{fig:QPIP1} we recall a protocol for verifying QFHE evaluation computations using just single-qubit computational and Hadamard basis measurements. This protocol is a $\secp$-wise parallel repetition of the quantum sampling verification protocol from \cite{Chung2020ConstantroundBC} applied to QFHE evaluation, which was also used in \cite{10.1007/978-3-030-90459-3_1}.

\begin{definition}
Fix a security parameter $\secp$ and keys $(\pk,\sk) \in \Gen(1^\secp)$. For $b \in \{0,1\}$, let $\mathsf{Maj}[\sk,b]$ be the set of sets of $\secp$ ciphertexts $\{\ct_i\}_{i \in [\secp]}$ such that for at least $\secp/2 + 1$ ciphertexts $\ct_i$, it holds that $\Dec(\sk,\ct_i) = b$.
\end{definition} 

\protocol{$\text{QPIP}_1$ protocol}{$\text{QPIP}_1$ protocol for verifying a QFHE evaluation.}{fig:QPIP1}{
\textbf{Common inputs}
\begin{itemize}
    \item QFHE ciphertext $\ct$
    \item Quantum circuit $Q$
    \item An X-Z local Hamiltonian $H_{\ct,Q} = \sum_k \alpha_k H_k$. Let $p_k = |\alpha_k|/\sum_k |\alpha_k|$ for each $k$ and let $P$ be the corresponding probability distribution over indices $k$. Let $\epsilon$ be a constant used for the verification threshold.
\end{itemize}
\textbf{Parameters}
\begin{itemize}
    %\item $T = T(\secp):$ number of qubits in history state $\ket{\psi_{\ct,Q}^{\mathsf{hist}}}$
    %\item $R \coloneqq R(\secp):$ number of parallel repetitions
    \item $n \coloneqq n(\secp):$ number of copies of $\ket{\psi_{\ct,Q}^{\mathsf{hist}}}$ per repetition
    \item $m \coloneqq m(\secp):$ number of Hamiltonian terms to measure per repetition
\end{itemize}
\textbf{Protocol}
\begin{itemize}
    \item The prover prepares $\secp \cdot n$ copies of $\ket{\psi_{\ct,Q}^{\mathsf{hist}}}$ and sends all copies to the verifier.
    \item The verifier does the following. For each $i \in [\secp]$:
    \begin{itemize}
        \item Sample a uniformly random $S_i \coloneqq (T_i \cup \{s_i\}) \subset [(i-1) \cdot n)+1,\dots,i \cdot n]$ of size $m+1$, where $T_i$ has size $m$.
        \item For each $j \in T_i$, sample $k[i,j]$ according to probability distribution $P$, and measure the $(i-1)n + j$ copy of $\ket{\psi_{\ct,Q}^{\mathsf{hist}}}$ with $H_{k[i,j]}$. Let $y[i,j] \in \{+1,-1\}$ be the result of this measurement multiplied by $\mathsf{sgn}(\alpha_{k[i,j]})$.
        \item Measure the ``output register'' qubits of the $(i-1)n + s_i$ copy of $\ket{\psi_{\ct,Q}^{\mathsf{hist}}}$ in the computational basis to obtain a classical string $\widetilde{\ct}_i$.
        \item If $\sum_j y[i,j] < (\frac{1}{2}+\epsilon) m$, then abort and output $\bot$.
    \end{itemize}
    \item If the verifier did not abort, output $(\top,\{\widetilde{\ct}_i\}_{i \in [\secp]})$.
\end{itemize}}

\begin{importedtheorem}[\cite{Chung2020ConstantroundBC,10.1007/978-3-030-90459-3_1}]
There exists a family of X-Z local Hamiltonians $\{H_{\ct,Q}\}_{\ct,Q}$ and polynomials $n(\secp),m(\secp)$ such that for any family of keys $\{(\pk_\secp,\sk_\secp) \in \Gen(1^\secp)\}_{\secp \in \bbN}$, inputs $\{x_\secp\}_{\secp \in \bbN}$, circuits $\{Q_\secp\}_{\secp \in \bbN}$, ciphertexts $\{\ct_\secp \in \Enc(\pk_\secp,x_\secp)\}_{\secp \in \bbN}$, and states $\{\ket{\psi_\secp}\}_{\secp \in \bbN}$, the following holds with probability $1-\negl(\secp)$. On input $\ket{\psi_\secp}$, the verifier in \proref{fig:QPIP1} either outputs $\bot$ or $(\top,\{\widetilde{\ct}_i\}_{i \in [\secp]})$ such that $\{\widetilde{\ct}_i\}_{i \in [\secp]} \in \mathsf{Maj}[\sk_\secp,Q_\secp(x_\secp)]$.
\end{importedtheorem}

\newpage

Next, we take an abstract view of \proref{fig:QPIP1}, which will useful for building on top of it. Based on $(\ct,Q)$, the prover prepares a state $\ket{\psi}$ and sends it to the verifier. Then, the verifier samples a string of bases $h \in \{0,1\}^{\ell(\secp)}$ for some polynomial $\ell(\secp)$, where each 0 corresponds the computational basis and each 1 corresponds to the Hadamard basis, and measures $\ket{\psi}$ in the bases specified by $h$.\footnote{In \proref{fig:QPIP1} the verifier actually does not measure every qubit sent by the prover, but for these qubits we can say the verifier measures in, say, the computational basis and then ignores the result.} Finally, the verifier applies a (classical) verification function to some substring of $h$ to obtain $\top$ or $\bot$. In the case of $\top$, the verifier outputs the remaining bits of $h$, which are parsed a set of ciphertexts $\{\widetilde{\ct}_i\}_{i \in [\secp]}$. This abstract view of the protocol is formalized in \cref{fig:abstract-QPIP1}.

\protocol{Abstracted $\text{QPIP}_1$ protocol $(\cP^\QV,\cV_\Gen^\QV,\cV_\Ver^\QV)$}{An abstract view of the $\text{QPIP}_1$ protocol for verifying QFHE evaluation.}{fig:abstract-QPIP1}{

\textbf{Common inputs}
\begin{itemize}
    \item QFHE ciphertext $\ct$
    \item Quantum circuit $Q$
\end{itemize}

\textbf{Parameters}
\begin{itemize}
    \item $\ell \coloneqq \ell(\secp):$ number of qubits in the prover's state
    %\item $R \coloneqq R(\secp):$ number of output ciphertexts
\end{itemize}

\textbf{Prover's computation}

\begin{itemize}
    \item $\cP^\QV(\ct,Q) \to \ket{\psi_{\ct,Q}}:$ on input a ciphertext $\ct$ and a quantum circuit $Q$, the prover prepares a state $\ket{\psi_{\ct,Q}}$ on $\ell$ qubits, and sends it to the verifier.
\end{itemize}

\textbf{Verifier's computation}

\begin{itemize}
    \item $\cV_\Gen^\QV(\ct,Q) \to (h,W):$ on input a ciphertext $\ct$ and a quantum circuit $Q$, the first verifier algorithm samples a string $h \in \{0,1\}^\ell$ and a subset $W \subset [\ell]$ with the property that for all $i \in W$, $h_i = 0$.
    \item Sample $c \gets M_h(\ket{\psi_{\ct,Q}})$ to obtain a string of measurement results $c \in \{0,1\}^\ell$. Define $c_\Ver$ to be the substring $\{c_i\}_{i \in [\ell] \setminus W}$ and define $c_\Out$ to be the substring $\{c_i\}_{i \in W}$.
    \item $\cV_\Ver^\QV(h,c_\Ver) \to \{\top,\bot\}:$ on input the string of bases $h$ and the substring of measurement results $c_\Ver$, the second verification algorithm outputs $\top$ or $\bot$.
    \item If $\top$, output $(\top,c_\Out)$, where $c_\Out$ is parsed as $\{\widetilde{\ct}_i\}_{i \in [\secp]}$, and otherwise output $\bot$.
\end{itemize}

}


\newpage
\fi

\subsection{Two-message classical verification}\label{subsec:2-message}

Next, we use Mahadev's measurement protocol \cite{FOCS:Mahadev18a} to make the verifier fully classical. We parallel repeat the protocol and apply Fiat-Shamir to make it non-interactive, following \cite{TCC:ACGH20,TCC:ChiChuYam20,10.1007/978-3-030-90459-3_1}. Finally, we add an ``output'' algorithm that takes as input the secret key $\sk_\QFHE$ of the QFHE scheme. 

Let $(\TCF.\Gen, \TCF.\Eval, \TCF.\Invert, \TCF.\Ch, \TCF.\IsValid)$ be a dual-mode randomized trapdoor claw-free hash function (\cref{def:clawfree}). The protocol is described \proref{fig:CVQC} and \proref{fig:CVQC2}.



\protocol{Classical verification protocol $\Pi^\CV = (\cP_\Prep^\CV,\cV^\CV_\Gen,\cP_\Prove^\CV,\cV^\CV_\Ver,\cV^\CV_\Out)$}{Two-message protocol for verifying QFHE evaluation with a classical verifier.}{fig:CVQC}{
\textbf{Common inputs}: QFHE ciphertext $\ct$, quantum circuit $Q$, random oracle $H: \{0,1\}^* \to \{0,1\}^{\log\binom{r}{k}}$.\\


\textbf{Parameters}: number of parallel repetitions $r \coloneqq r(\secp)$, number of Hadamard rounds $k \coloneqq k(\secp)$, and number of qubits in each repetition $\ell \coloneqq \ell(\secp)$.\\

\textbf{Protocol}
\begin{itemize}
    \item $\cP_\Prep^\CV(\ct,Q) \to (\sM_1,\dots,\sM_r)$:
    \begin{itemize}
        \item For each $i \in [r]$, prepare the state $\ket{\psi_{\ct,Q}} \gets \cP^\QV(\ct,Q)$, which we write as 
            \[\ket{\psi_{\ct,Q}} \coloneqq \sum_{m \in \{0,1\}^\ell}\alpha_m\ket{m}^{\sB_i}.\]
    \end{itemize}
    \item $\cV_\Gen^\CV(\ct,Q) \to (\pp,\sparam)$: 
    \begin{itemize}
        \item For each $i \in [r]$, sample $(h_i,W_i) \gets \cV^\QV_\Gen(\ct,Q)$ and $\{(\pk_{i,j},\sk_{i,j}) \gets \TCF.\Gen(1^\secp,h_{i,j})\}_{j \in [\ell]}$, and set \[\pp \coloneqq \{\pk_{i,j}\}_{i \in [r],j \in [\ell]},  \ \ \, \sparam \coloneqq (\{h_i,W_i,\{\sk_{i,j}\}_{j \in [\ell]}\}_{i \in [r]}).\]
    \end{itemize}
    \item $\cP_\Prove^\CV(\sB_1,\dots,\sB_r,\pp) \to (\sB_1,\dots,\sB_r,\{y_{i,j},z_{i,j}\}_{i \in [r], j \in [\ell]})$:
    \begin{itemize}
        \item For each $i \in [r]$, apply $\TCF.\Eval[\pk_{i,j}]$ from register $\sB_{i,j}$ to registers $(\sB_{i,j},\sX_{i,j},\sY_{i,j})$ for each $j \in [\ell]$, resulting in the state
            \[\sum_{m \in \{0,1\}^\ell}\alpha_m\ket{m}^{\sB_i}\ket{\psi_{\pk_{i,1},m_1}}^{\sX_{i,1},\sY_{i,1}},\dots,\ket{\psi_{\pk_{i,\ell},m_\ell}}^{\sX_{i,\ell},\sY_{i,\ell}},\]
            and measure registers $\sY_{i,1},\dots,\sY_{i,\ell}$ in the computational basis to obtain strings $y_{i,1},\dots,y_{i,\ell}$.
        \item Compute $T \coloneqq H(y_{1,1},\dots,y_{r,\ell})$, which is parsed as a string $T \in \{0,1\}^r$ with Hamming weight $k$.
        \item For each $i: T_i = 0$, measure registers $\sX_{i,1},\dots,\sX_{i,\ell}$ in the computational basis to obtain strings $z_{i,1},\dots,z_{i,\ell}$.
        \item For each $i: T_i = 1$, apply $J(\cdot)$ coherently to each register $\sX_{i,1},\dots,\sX_{i,\ell}$ and then measure registers $\sX_{i,1},\dots,\sX_{i,\ell}$ in the Hadamard basis to obtain strings $z_{i,1},\dots,z_{i,\ell}$.
        %\item Set \[\pi \coloneqq (\{y_{i,j}\}_{i \in [r],j \in [\ell]},\{(m_{i,j},x_{i,j})\}_{i \in T, j \in [\ell]},\{(e_{i,j},d_{i,j})\}_{i \in [n] \setminus T, j \in [\ell]}).\]
    \end{itemize}
    \item The prover measures registers $\{\sB_{i,j}\}_{i: T_i = 0, j \in [\ell]}$ in the computational basis to obtain bits $\{b_{i,j}\}_{i: T_i = 0, j \in [\ell]}$ and measures registers $\{\sB_{i,j}\}_{i: T_i = 1, j \in [\ell]}$ in the Hadamard basis to obtain bits $\{b_{i,j}\}_{i: T_i = 1, j \in [\ell]}$. The final proof is set to \[\pi \coloneqq \{y_{i,j},b_{i,j},z_{i,j}\}_{i \in [r], j \in [\ell]}.\]
\end{itemize}
}

\protocol{Classical verification protocol $\Pi^\CV = (\cP_\Prep^\CV,\cV^\CV_\Gen,\cP_\Prove^\CV,\cV^\CV_\Ver,\cV^\CV_\Out)$ (cont.)}{Two-message protocol for verifying QFHE evaluation with a classical verifier.}{fig:CVQC2}{

\textbf{Protocol (cont.)}
\begin{itemize}
    \item $\cV_\Ver^\CV(\sparam,\pi) \to \{\bot\} \cup \{(\top,\{\{\widetilde{\ct}_{i,s}\}_{s \in [\secp]}\}_{i \in [r] \setminus T})\}$:
    \begin{itemize}
        \item Compute $T \coloneqq H(y_{1,1},\dots,y_{r,\ell})$.
        \item For each $i: T_i = 0$ and $j \in [\ell]$, compute $\TCF.\Ch(\pk_{i,j},b_{i,j},z_{i,j},y_{i,j})$. If any are $\bot$, then abort and output $\bot$.
        \item For each $i: T_i = 1$, do the following.
        \begin{itemize}
            \item For each $j \in [\ell]$: If $h_{i,j} = 0$, compute $\TCF.\Invert(0,\sk_{i,j},y_{i,j})$, abort if the output is $\bot$ and otherwise parse the output as $(c_{i,j},x_{i,j})$. If $h_{i,j} = 1$, compute $\TCF.\Invert(1,\sk_{i,j},y_{i,j})$, abort if the output is $\bot$ and otherwise parse the output as $(0,x_{i,j,0}),(1,x_{i,j,1})$. Then, check $\TCF.\IsValid(x_{i,j,0},x_{i,j,1},z_{i,j})$ and abort if the result is $\bot$. Finally, set $c_{i,j} \coloneqq b_{i,j} \oplus z_{i,j} \cdot (J(x_{i,j,0}) \oplus J(x_{i,j,1}))$.
            \item Let $c_i  = (c_{i,1},\dots,c_{i,\ell})$, and define $c_{i,\Ver}$ and $c_{i,\Out}$ as in $\Pi^\QV$, based on the set $W_i$. Compute $\cV_\Ver^\QV(h_i,c_{i,\Ver})$ and abort if the result is $\bot$.
        \end{itemize}
        \item Parse each $c_{i,\Out}$ for $i: T_i = 1$ as a set of ciphertexts $\{\widetilde{\ct}_{i,s}\}_{s \in [\secp]}$ and output \[(\top,\{\{\widetilde{\ct}_{i,s}\}_{s \in [\secp]}\}_{i: T_i = 1}).\]
    \end{itemize}
    \item $\cV^\CV_\Out(\sk_\QFHE,\{\{\widetilde{\ct}_{i,s}\}_{s \in [\secp]}\}_{i: T_i = 1}) \to \{0,1\}$: 
    \begin{itemize}
        \item Use $\sk_\QFHE$ to decrypt each $\widetilde{\ct}_{i,s}$, obtaining $\{\{z_{i,s}\}_{s \in [\secp]}\}_{i: T_i = 1}$, and output the bit $\mathsf{maj}_{i: T_i = 1}\{\mathsf{maj}_{s \in [\secp]}\{z_{i,s}\}\}$.
    \end{itemize}
\end{itemize}
}


Now, we introduce some notation needed for describing the security properties of this protocol. 

\begin{itemize}
    \item Given parameters $(\pp,\sparam)$, we define a subset of indices $W \subset [r \cdot \ell]$ by $D \coloneqq \{W_i\}_{i \in [r]}$. That is, $W$ is all of the ``output'' indices across the parallel repetitions. Note that, if $t = t(\secp)$ is the size of an QFHE ciphertext, then the size of $W$ is $r \cdot \secp \cdot t$. In what follows, we will define incompatible predicates (\cref{def:incompatible-predicates}) on $W$, parameterized by a QHFE secret key $\sk_\QFHE$ and a bit $b$. 
    \item For any QFHE secret key $\sk_\QFHE$ and bit $b \in \{0,1\}$, we define $D_{\inside}[\sk_\QFHE,b]$ to consists of $w \in \{0,1,*\}^{|W|}$ such that, when $w$ is parsed as $(w_1,\dots,w_r)$ for $w_i \in \{0,1\}^{\secp \cdot t}$, there are at least $3/4$ fraction of $w_i$ that are such that $w_i \in \{0,1\}^{\secp \cdot t}$ and, when parsed as $\{\widetilde{\ct}_s\}_{s \in [\secp]}$, it holds that $\{\widetilde{\ct}_s\}_{s \in [\secp]} \in \mathsf{Maj}[\sk_\QFHE,b]$. 
    \item For any QFHE secret key $\sk_\QFHE$ and bit $b \in \{0,1\}$, we define $D_{\out}[\sk_\QFHE,b]$ to consists of $w \in \{0,1,*\}^{|W|}$ such that, when $w$ is parsed as $(w_1,\dots,w_r)$ for $w_i \in \{0,1\}^{\secp \cdot t}$, there are at least $1/3$ fraction of $w_i$ that are such that $w_i \in \{0,1\}^{\secp \cdot t}$ and, when parsed as $\{\widetilde{\ct}_s\}_{s \in [\secp]}$, it holds that $\{\widetilde{\ct}_s\}_{s \in [\secp]} \notin \mathsf{Maj}[\sk_\QFHE,b]$. 
    %\item For $b \in \{0,1\}$, say that $w \in D_{\out,b}$ if there are at least $1/3$ fraction of $w_i$ that are all bit strings $\in \{0,1\}^{\secp \cdot t}$ and, when parsed as $\{\widetilde{\ct}_s\}_{s \in [\secp]}$, it holds that $\{\widetilde{\ct}_s\}_{s \in [\secp]} \notin \mathsf{Maj}[\sk_\QFHE,b]$. 
    \item It is clear that for any $\sk_\QFHE$ and $b \in \{0,1\}$, $D_{\inside}[\sk_\QFHE,b]$ and $D_{\out}[\sk_\QFHE,b]$ are incompatible predicates.
    \item For a proof $\pi = \{y_{i,j},b_{i,j},z_{i,j}\}_{i \in [r], j \in [\ell]}$ generated during $\Pi^\CV$, define $\mathsf{TestRoundOutputs}[\sparam](\pi) \in \{0,1,*\}^{|W|}$ as follows. $\mathsf{TestRoundOutputs}[\sparam](\pi)$ is a string consisting of $r$ substrings, where the $i$'th substring consists of all $*$ for each $i: T_i = 1$, and consists of the bits $\{b_{i,j}\}_{j \in W_j}$ for each $i: T_i = 0$. We include $\sparam$ in the description of $\mathsf{TestRoundOutputs}[\sparam]$ since the functionality depends on $\{W_i\}_{i \in [r]}$, which are part of $\sparam$.
\end{itemize}

Then, $\Pi^\CV$ satisfies the following three properties. The proofs of these lemmas mostly follow from the prior work of \cite{10.1007/978-3-030-90459-3_1}, and we show this formally in \cref{sec:appendix-CVQC}.

\begin{lemma}[Soundness]\label{lemma:soundness}
$\Pi^\CV$ with $r(\secp) = \secp^2 + \secp$ and $k(\secp) = \secp^2$ satisfies \emph{soundness}, which stipulates that for any $(\pk_\QFHE,\sk_\QFHE) \in \Gen(1^\secp), \ct \in \Enc(\pk_\QFHE,x), Q$, and QPT adversarial prover $\cA$, it holds that 
    \[\Pr\left[\begin{array}{l}\cV_\Ver^\CV(\sparam,\pi) = (\top,\{\{\widetilde{\ct}_{i,s}\}_{s \in [\secp]}\}_{i: T_i = 1})\\ \wedge \ \cV^\CV_\Out(\sk_\QFHE,\{\{\widetilde{\ct}_{i,s}\}_{s \in [\secp]}\}_{i: T_i = 1}) = 1-Q(x)\end{array} : \begin{array}{r}(\pp,\sparam) \gets \cV^\CV_\Gen(\ct,Q) \\ \pi \gets \cA(\ct,Q,\pp)\end{array}\right] = \negl(\secp).\]
\end{lemma}

\begin{lemma}[$D_{\inside}{[}\sk_\QFHE,Q(x){]}$ if accept]\label{lemma:Q-in}
$\Pi^\CV$ with $r(\secp) = \secp^2 + \secp$ and $k(\secp) = \secp^2$ satisfies the following property. For any $(\pk_\QFHE,\sk_\QFHE) \in \Gen(1^\secp), \ct \in \Enc(\pk_\QFHE,x), Q$, and QPT adversarial prover $\cA$, it holds that 
        \[\Pr\left[\begin{array}{l}\cV^\CV_\Ver(\sparam,\pi) = (\top,\cdot) \\ \wedge \ w \notin D_{\inside}[\sk_\QFHE,Q(x)]\end{array} : \begin{array}{r}(\pp,\sparam) \gets \cV^\CV_\Gen(\ct,Q) \\ \pi \gets \cA(\ct,Q,\pp) \\ w \coloneqq \mathsf{TestRoundOutputs}[\sparam](\pi)\end{array}\right] = \negl(\secp).\]
\end{lemma}

\begin{lemma}[$D_{\out}{[}\sk_\QFHE,Q(x){]}$ if accept $1-Q(x)$]\label{lemma:Q-out}
$\Pi^\CV$ with $r(\secp) = \secp^2 + \secp$ and $k(\secp) = \secp^2$ satisfies the following property. For any $(\pk_\QFHE,\sk_\QFHE) \in \Gen(1^\secp), \ct \in \Enc(\pk_\QFHE,x), Q$, and QPT adversarial prover $\cA$, it holds that 
        \[\Pr\left[\begin{array}{l} \cV^\CV_\Ver(\sparam,\pi) = (\top,\{\widetilde{\ct}_{i,s}\}_{s \in [\secp]}\}_{i: T_i = 1})\\ \wedge \ \cV^\CV_\Out(\sk_\QFHE,\{\{\widetilde{\ct}_{i,s}\}_{s \in [\secp]}\}_{i: T_i = 1}) = 1-Q(x)\\ \wedge \ w \notin D_{\out}[\sk_\QFHE,Q(x)]\end{array} : \begin{array}{r}(\pp,\sparam) \gets \cV^\CV_\Gen(\ct,Q) \\ \pi \gets \cA(\ct,Q,\sparam) \\ w \coloneqq \mathsf{TestRoundOutputs}[\sparam](\pi)\end{array}\right] = \negl(\secp).\]
\end{lemma}

Note that in this final lemma, $\cA$ is even given access to $\sparam$.

%\begin{proof}
%\james{TODO: This follows from the random oracle.}
%\end{proof}




%\begin{definition}
%For a proof $\pi$ generated during $\proref{fig:CVQC}$, define $\mathsf{TestOutput}(\pi) = \{\{\widetilde{\ct}_{i,s}\}_{s \in [\secp]}\}_{i \in T}$ by, for each $i \in T$, parsing $\{m_{i,j}\}_{j \in W_i}$ as a set of ciphertexts $\{\widetilde{\ct}_{i,s}\}_{s \in [\secp]}$. 
%\end{definition}
\iffalse
\begin{itemize}
    \item \textbf{Soundness:} For any $\ct \in \Enc(\pk_\QFHE,x),Q$ and QPT adversarial prover $\cA$, it holds that 
    \[\Pr\left[\begin{array}{l}(\top,\{\{\widetilde{\ct}_{i,s}\}_{s \in [\secp]}\}_{i \in [n] \setminus T}) \gets \cV_\Ver^\CV(\sparam,\pi) \\ \wedge \ \cV^\CV_\Out(\sk_\QFHE,\{\{\widetilde{\ct}_{i,s}\}_{s \in [\secp]}\}_{i \in [n] \setminus T}) = 1-Q(x)\end{array} : \begin{array}{r}(\pp,\sparam) \gets \cV^\CV_\Gen(\ct,Q) \\ \pi \gets \cA(\ct,Q,\pp)\end{array}\right] = \negl(\secp).\]
    \james{This is already shown in [Bar21], by the security of QV protocol + [Mah18] measurement protocol + [ACGH21/Bar21] parallel repetition + Fiat-Shamir}
    
    \item \textbf{Extra property:} There exist $n' = n'(\secp)$ and $n'' = n''(\secp)$ where $n' + T - n'' > n$ such that the following hold.
    \begin{enumerate}
        \item For any $\ct \in \Enc(\pk_\QFHE,x),Q$ and QPT adversarial prover $\cA$, it holds that 
        \[\Pr\left[\begin{array}{l}(\top,\cdot) \gets \cV^\CV_\Ver(\sparam,\pi) \\ \wedge \ \nexists \ n' \text{ indices } i \in T \text{ s.t. } \mathsf{CT}_i \in \mathsf{Maj}[Q(x)]\end{array} : \begin{array}{r}(\pp,\sparam) \gets \cV^\CV_\Gen(\ct,Q) \\ \pi \gets \cA(\ct,Q,\pp) \\ \{\mathsf{CT}_i\}_{i \in T} \coloneqq \mathsf{TestOutput}(\pi)\end{array}\right] = \negl(\secp).\]
        \james{The corresponding claim for the Hadamard rounds is already implicitly shown in [Bar21], and we can use CI of the random oracle to establish this for the test rounds.}
        \item For any $\ct \in \Enc(\pk_\QFHE,x),Q$ and QPT adversarial prover $\cA$, it holds that 
        \[\Pr\left[\begin{array}{l}(\top,\{\widetilde{\ct}_{i,s}\}_{s \in [\secp]}\}_{i \in [n] \setminus T}) \gets \cV^\CV_\Ver(\sparam,\pi) \\ \wedge \ \cV^\CV_\Out(\sk_\QFHE,\{\{\widetilde{\ct}_{i,s}\}_{s \in [\secp]}\}_{i \in [n] \setminus T}) = b\\ \wedge \ \exists \ n'' \text{ indices } i \in T \text{ s.t. } \mathsf{CT}_i \in \mathsf{Maj}[1-b]\end{array} : \begin{array}{r}(\pp,\sparam) \gets \cV^\CV_\Gen(\ct,Q) \\ \pi \gets \cA(\ct,Q,\sparam,\sk_\QFHE) \\ \{\mathsf{CT}_i\}_{i \in T} \coloneqq \mathsf{TestOutput}(\pi)\end{array}\right] = \negl(\secp).\]
        \james{This follows directly from CI of the random oracle.}
    \end{enumerate}
\end{itemize}
\fi



==> Unique-signature-tokens.tex <==
% !TEX root = main.tex
\section{Strongly unforgeable signature tokens}\label{sec:sig-tokens}

\subsection{Definition}

A signature token scheme consists of algorithms $(\Gen,\Sign,\Verify)$ with the following syntax.

\begin{itemize}
    \item $\Gen(1^\secp,k) \to (\vk,\ket{\sk})$: The $\KeyGen$ algorithm takes as input the security parameter $1^\secp$ and an integer $k$ determining the message length, and outputs a public verification key $\vk$ and a quantum signing key $\ket{\sk}$.
    \item $\Sign(m,\ket{\sk}) \to \sigma$: The $\Sign$ algorithm takes as input a message $m \in \{0,1\}^{k}$ and the signing key $\ket{\sk}$, and outputs a signature $\sigma$.
    \item $\Verify(\vk,m,\sigma) \to \{\top,\bot\}$: The $\Verify$ algorithm takes as input a verification key $\vk$, a message $m$, and a signature $\sigma$, and outputs $\top$ or $\bot$.
\end{itemize}

In this paper, it suffices to use a signature token scheme in the \emph{oracle model}, where the adversary is not given $\vk$, but rather has oracle access to its functionality. We say that a signature token scheme is \emph{1-strongly-unforgeable} if the following holds.

\begin{definition}\label{def:unforgeability}
A signature token scheme $(\KeyGen,\Sign,\Verify)$ satisfies \emph{1-strong-unforgeability} if for any QPT adversary $\cA$,

\[\Pr\left[\begin{array}{c} (m_0,\sigma_0) \neq (m_1,\sigma_1) \\ \wedge \ \Verify(\vk,m_0,\sigma_0) = \top \\ \wedge \ \Verify(\vk,m_1,\sigma_1) = \top\end{array} : \begin{array}{r} (\vk,\ket{\sk}) \gets \KeyGen(1^\secp,k) \\ (m_0,\sigma_0,m_1,\sigma_1) \gets \cA^{\Verify(\vk,\cdot,\cdot)}(\ket{\sk}) \end{array}\right] = \negl(\secp).\]
\end{definition}

\subsection{Construction}

We show that the signature token construction from \cite{https://doi.org/10.48550/arxiv.1609.09047}, which was shown to be 1-unforgeable, in fact satisfies 1-\emph{strong}-\emph{unforeability}. The construction for signing a single bit is as follows. Repeating it $k$ times produces a signature token scheme for $k$-bit messages.

\begin{itemize}
    \item $\Gen(1^\secp)$: Sample a uniformly random $\secp/2$ dimensional subspace $S$ of $\bbF_2^\secp$. Let $\vk \coloneqq S$ and $\ket{\sk} \coloneqq \ket{S}$.
    \item $\Sign(b,\ket{\sk})$: If $b = 0$, measure $\ket{\sk}$ in the computational basis to obtain a string $\sigma$. Otherwise, if $b = 1$, apply $H^{\otimes n}$ to $\ket{\sk}$ and then measure in the computational basis to obtain a string $\sigma$.
    \item $\Verify(S,b,\sigma)$: If $b = 0$, output $\top$ if $\sigma \in S \setminus \{0^\secp\}$ and if $b = 1$, output $\top$ if $\sigma \in S^\bot \setminus \{0^\secp\}$. Otherwise, output $\bot$.
\end{itemize}

\begin{theorem}
The above signature token construction satisfies 1-strong-unforgeability.
\end{theorem}

Since the proof of this theorem closely follows \cite{https://doi.org/10.48550/arxiv.1609.09047} with one tweak, we defer it to \cref{sec:appendix-tokens}.

==> commitment-old.tex <==
\section{Pauli Functional Commitments}\label{sec:SSC}

\subsection{Definition}

A Pauli Functional Commitment is similar to a standard bit commitment scheme with a classical receiver. However, when used to commit to a qubit $\ket{\psi} = \alpha_0\ket{0} + \alpha_1\ket{1}$ in superposition, it supports the ability to open to a either a \emph{standard} or \emph{Hadamard} basis measurement of $\ket{\psi}$. Beyond this functionality, a Pauli functional commitment should satisfy some notion of binding to a classical bit.

The syntax of a Pauli functional commitment is given below. We present the syntax in the \emph{oracle model}, where the committer obtains access to an efficient classical oracle $\cCK$ as part of its commitment key. Such a scheme can be heuristically instantiated in the plain model by using a post-quantum indistinguishability obfuscator to obfuscate this oracle. We also specify that the remainder of the commitment key is a quantum state $\ket{\ck}$, but note that this is not inherent.
 
%Moreover, we allow the honest Commit algorithm and the adversary in the Commit stage to have access to classical oracles that hard-code the receiver's secret decoding key, and allow to decode the results of standard and Hadamard basis measurements. Crucially, we do not give the adversary in the Open stage access to the receiver's Hadamard measurement decoding functionality. 

\begin{definition}[Pauli Functional Commitment: Syntax]\label{def:PFC}
A Pauli functional commitment consists of six algorithms $(\Gen,\allowbreak\Com,\allowbreak\OpenZ,\allowbreak\OpenX,\allowbreak\DecZ,\allowbreak\DecX)$ with the following syntax.

\begin{itemize}
    \item $\Gen(1^\secp) \to (\dk,\ket{\ck},\cCK)$ is a QPT algorithm that takes as input the security parameter $1^\secp$ and outputs a classical decoding key $\dk$ and a quantum commitment key $(\ket{\ck},\cCK)$, where $\ket{\ck}$ is a quantum state on register $\sC$, and $\cCK$ is the description of a classical deterministic polynomial-time functionality $\cCK: \{0,1\}^* \to \{0,1\}^*$.
    %\item $\OZ[\dk]: \{0,1\}^* \to \{0,1\}^*$ is a (deterministic) polynomial-time classical functionality.
    %\item $\OX[\dk]: \{0,1\}^* \to \{0,1\}^*$ is a (deterministic) polynomial-time classical functionality.
    \item $\Com_b^{\cCK}(\ket{\ck}) \to (\sS,y)$ is a QPT algorithm that is parameterized by a bit $b$ and has oracle access to $\cCK$. It applies a map from register $\sC$ (initially holding the commitment key $\ket{\ck}$) to registers $(\sS,\sY)$ and then measures $\sY$ in the computational basis to obtain a classical string $y \in \{0,1\}^*$ and a left-over state on register $\sS$. We then write \[\Com^{\cCK} \coloneqq \ketbra{0}{0} \otimes \Com_0^{\cCK} + \ketbra{1}{1} \otimes \Com_1^{\cCK}\] to refer to the map that applies the  $\Com_b^{\cCK}$ map classically controlled on a single-qubit register $\sB$ to produce a state on registers $(\sB,\sS,\sY)$, and then measures $\sY$ in the computational basis to obtain a classical string $y$ along with a left-over quantum state on registers $(\sB,\sS)$.
    \item $\OpenZ(\sB,\sS) \to z$ is a QPT measurement on registers $(\sB,\sS)$ that outputs a classical string $z$.
    \item $\OpenX(\sB,\sS) \to z$ is a QPT measurement on registers $(\sB,\sS)$ that outputs a classical string $z$.
    \item $\DecZ(\dk,y,z) \to \{0,1,\bot\}$ is a classical deterministic polynomial-time algorithm that takes as input the decoding key $\dk$, a string $y$, and a string $z$, and outputs either a bit $b$ or a $\bot$ symbol.
    \item $\DecX(\dk,y,z) \to \{0,1,\bot\}$ is a classical deterministic polynomial-time algorithm that takes as input a the decoding key $\dk$, a string $y$, and a string $z$, and outputs either a bit $b$ or a $\bot$ symbol.
    %\item \textbf{Commitment.} $\Com_b^{\OpenZ[\dk],\OpenX[\dk]}$ is a polynomial-size unitary that operates on register $\sC$. It is parameterized by a bit $b$, and has access to the classical oracles $\OpenZ[\dk]$ and $\OpenX[\dk]$. Given a one-qubit register $\sB$, we also write \[\Com^{\OpenZ[\dk],\OpenX[\dk]} \coloneqq \ketbra{0}{0} \otimes \Com_0^{\OpenZ[\dk],\OpenX[\dk]} + \ketbra{1}{1} \otimes \Com_1^{\OpenZ[\dk],\OpenX[\dk]}\] to refer to the $(k+1)$-qubit unitary that applies the unitary $\Com_b^{\OpenZ[\dk],\OpenX[\dk]}$ to register $\sC$ classically controlled on register $\sB$.
\end{itemize}

\end{definition} 

%\begin{remark}
%It would also make sense to augment the output of $\Com_b$ with a classical string $y$, and have $\DecZ$ and $\DecX$ take $y$ as an additional input. This corresponds to the usual syntax of a commitment with classical receiver where $y$ would represent the classical commitment string and $\sS$ the left-over state of the committer. In the binding definition below, we would have included $y$ in the projections $\Pi_{\dk,y,0}$ and $\Pi_{\dk,y,1}$. Interestingly, in our construction, we do not need to include any string $y$ to obtain a binding commitment, so we omit it in the above definition. 
%\end{remark}

%\begin{definition}
%Given an $n$-qubit register $\sX$ and an $n$-bit string $h$, let $M_h(\sX)$ refer to the distribution over classical $n$-bit strings that results from measuring each qubit $i$ of $\sX$ in basis $h_i$, where 0 denotes the computational basis and 1 denotes the Hadamard basis. 
%\end{definition}

\begin{definition}[Pauli Functional Commitment: Correctness]\label{def:poc-correctness}
A Pauli functional commitment $(\Gen,\allowbreak\Com,\allowbreak\OpenZ,\allowbreak\OpenX,\allowbreak\DecZ,\allowbreak\DecX)$ is \emph{correct} if for any single-qubit (potentially mixed) state $\rho$ on register $\sB$, it holds that \[\Bigg|\Pr\left[1 \gets Z(\sB)\right] - \Pr\left[1 \coloneqq \DecZ(\dk,y,z) : \begin{array}{r}(\dk,\ket{\ck},\cCK) \gets \Gen(1^\secp) \\ (\sB,\sS,y) \gets \Com^{\cCK}(\sB,\ket{\ck}) \\ z \gets \OpenZ(\sB,\sS) \end{array}\right]\Bigg| = \negl(\secp),\]
and it holds that 
\[\Bigg|\Pr[1 \gets X(\sB)] - \Pr\left[1 \coloneqq \DecX(\dk,y,z) : \begin{array}{r}(\dk,\ket{\ck},\cCK) \gets \Gen(1^\secp) \\ (\sB,\sS,y) \gets \Com^{\cCK}(\sB,\ket{\ck}) \\ z \gets \OpenX(\sB,\sS) \end{array}\right]\Bigg| = \negl(\secp),\] where $Z(\sB)$ denotes the distribution over a bit that results from measuring $\sB$ in the standard basis, and  $X(\sB)$ denotes the distribution over a bit that results from measuring $\sB$ in the Hadamard basis.
\end{definition}


A Pauli functional commitment that satisfies \emph{reusable binding} allows the adversarial committer oracle access to the receiver's decoding functionalities. That is, the adversarial committer has oracle access to both $\DecZ(\dk,\cdot,\cdot)$ and $\DecX(\dk,\cdot,\cdot)$. However, to allow for the possibility of achieving a non-trivial binding property, we cannot give the adversary access to $\DecX(\dk,\cdot,\cdot)$ during the Open stage.

\begin{definition}[Pauli Functional Commitment: Reusable single-bit binding]\label{def:poc-single-bit-binding}
A Pauli functional commitment $(\Gen,\Com,\allowbreak\OpenZ,\allowbreak\OpenX,\allowbreak\DecZ,\allowbreak\DecX)$ satisfies $p$ \emph{reusable single-bit binding} for some $p = p(\secp)$ if the following holds. Given $\dk,y,$ and $b \in \{0,1\}$, let $\Pi_{\dk,y,b}$ be a projection onto strings $z$ such that $\DecZ(\dk,y,z) = b$. Consider any adversary $\{(\cC_\secp, \cU_\secp)\}_{\secp \in \bbN}$, where each $\cC_\secp$ is an oracle-aided quantum operation, each $\cU_\secp$ is an oracle-aided unitary, and each $(\cC_\secp,\cU_\secp)$ make at most $\poly(\secp)$ oracle queries. Then for any $b \in \{0,1\}$,

\[\Pr_{\dk,\ket{\ck},\cCK \gets \Gen(1^\secp)}\left[\bigg\|\Pi_{\dk,y,1-b}\cU_\secp^{\cCK,\DecZ[\dk]}\Pi_{\dk,y,b}\ket{\psi}\bigg\| \geq \frac{1}{2^{p(\secp)}} : (\ket{\psi},y) \gets \cC_\secp^{\cCK,\DecZ[\dk],\DecX[\dk]}(\ket{\ck})\right] = \negl(\secp),\] where $\DecZ[\dk]$ is the oracle implementing the classical functionality $\DecZ(\dk,\cdot,\cdot)$ and $\DecX[\dk]$ is the oracle implementing the classical functionality $\DecX(\dk,\cdot,\cdot)$.

%\[\Pr_{\dk,\ket{\ck} \gets \Gen(1^\secp)}\left[\bra{\psi}\Pi_{\dk,0}\left(\cU^{\OZ[\dk]}\right)^\dagger\Pi_{\dk,1}\left(\cU^{\OZ[\dk]}\right)\Pi_{\dk,0}\ket{\psi} \geq \frac{1}{2^{p(\secp)}} : \ket{\psi} \gets \cC^{\OZ[\dk],\OX[\dk]}(\ket{\ck})\right] = \negl(\secp).\]
\end{definition}

%\begin{remark}
%Note that we do not allow $\cU_\secp$ to have access to $\cC$ during the Open phase. This seems problematic since $\cC$ is actually used by the honest Commit algorithm, and it is necessary for the correctness of the functional commitment. Indeed, naively instantiating $\cC$ using post-quantum indistinguishability obfuscation would not result in a candidate plain model construction, since there would then be no way to restrict $\cU_\secp$'s access to $\cC$. 

%However, when we eventually use this commitment scheme in a larger context, we will make use of signature tokens to ensure that $\cC_\secp$ may have access to $\cC$, but $\cU_\secp$ cannot. This will result in a protocol that \emph{can} be heuristically instantiated with post-quantum indistinguishability obfuscation.
%\end{remark}

Next, we extend the above single-bit binding property to a notion of string, or \emph{predicate}, binding, which is similar to the notion defined in \cite{AC:Yan21}.

\begin{definition}[Incompatible predicates]\label{def:incompatible-predicates}
Two sets of strings $W_0,W_1 \subset \{0,1,*\}^m$ are $m$-bit \emph{incompatible predicates} if for any $w_0 \in W_0$ and $w_1 \in W_1$, there exists $i \in [m]$ such that $w_{0,i},w_{1,i} \neq *$ and $w_{0,i} \neq w_{1,i}$.
\end{definition}

\begin{definition}[Pauli Functional Commitment: Reusable predicate binding]\label{def:predicate-binding} A Pauli functional commitment $(\Gen,\allowbreak\Com,\allowbreak\OpenZ,\allowbreak\OpenX,\allowbreak\DecZ,\allowbreak\DecX)$ satisfies $(m,p)$ \emph{reusable predicate binding} for some $m = m(\secp), p = p(\secp)$ if the following holds for any $m$-bit incompatible predicates $W_0,W_1$. Given a set of $m$ verification keys $\bdk = (\dk_1,\dots,\dk_m)$, and $m$ strings $\by = (y_1,\dots,y_m)$, define \[\Pi_{\bdk,\by,W_0} \coloneqq \sum_{w_0 \in W_0} \left(\bigotimes_{i: w_{0,i} \neq *}\Pi_{\dk_i,y_i,w_{0,i}} \right), \ \ \ \Pi_{\bdk,\by,W_1} \coloneqq \sum_{w_1 \in W_1} \left(\bigotimes_{i: w_{1,i} \neq *}\Pi_{\dk_i,y_i,w_{1,i}} \right).\]  Consider any adversary $\{(\cC_\secp, \cU_\secp)\}_{\secp \in \bbN}$, where each $\cC_\secp$ is an oracle-aided quantum operation, each $\cU_\secp$ is an oracle-aided unitary, and each $(\cC_\secp,\cU_\secp)$ make at most $\poly(\secp)$ oracle queries. Then,

\begin{align*}\Pr_{\{\dk_i,\ket{\ck_i},\cCK_i \gets \Gen(1^\secp)\}_{i \in [m]}}&\left[\bigg\|\Pi_{\bdk,\by,W_1}\cU_\secp^{\cCK,\DecZ[\bdk]}\Pi_{\bdk,\by,W_0}\ket{\psi}\bigg\| \geq \frac{1}{2^{p(\secp)}} : (\ket{\psi},\by) \gets \cC_\secp^{\cCK,\DecZ[\bdk],\DecX[\bdk]}(\ket{\mathbf{\bck}})\right] \\ &= \negl(\secp), \end{align*}


%\begin{align*}\Pr_{\{\dk_i,\ket{\ck_i} \gets \Gen(1^\secp)\}_{i \in [m]}}&\left[\bra{\psi}\Pi_{\dk,W_0}\left(U_\Open^{\OZ[\dk]}\right)^\dagger\Pi_{\dk,W_1}\left(U_\Open^{\OZ[\dk]}\right)\Pi_{\dk,W_0}\ket{\psi} \geq \frac{1}{2^{p(\secp)}} : \ket{\psi} \coloneqq U_\Com^{\OZ[\dk],\OX[\dk]}(\ket{\mathbf{\ck}})\right] = \negl(\secp), \end{align*} 

where $\ket{\bck} = (\ket{\ck_1},\dots,\ket{\ck_m})$, $\cCK$ is the collection of oracles $\cCK_1,\dots,\cCK_m$, $\DecX[\bdk]$ is the collection of oracles $\DecX[\dk_1],\dots,\DecX[\dk_m]$, and $\DecZ[\bdk]$ is the collection of oracles $\DecZ[\dk_1],\dots,\DecZ[\dk_m]$. We say that a Pauli functional commitment satisfies $m$ \emph{reusable predicate binding} if it satisfies $(m,p)$ \emph{reusable predicate binding} for any $p = O(\log(\secp))$.
\end{definition}

We show that single-bit binding generically implies predicate binding for an appropriate setting of parameters. However, to show predicate binding for $m$-bit messages, we need to assume single-bit binding with parameter $p \geq 4m$, meaning that when $m = \poly(\secp)$, the single-bit scheme must be ``exponentially'' secure. This is good enough for us, because we can construct such a scheme in the oracle model. We also note that the question of whether this exponential loss is necessary was recently addressed by \cite{AC:Yan21}, who showed how to take just a polynomial loss is certain specific settings. 

\begin{lemma}
Any Pauli functional commitment that satisfies $p$ \emph{reusable single-bit binding} for $p(\secp) = \poly(\secp)$ also satisfies $m$ \emph{reusable predicate binding} for any $m$ such that $p \geq 4m$.
\end{lemma}

\begin{proof}
Suppose that the commitment does not satisfy $m$ reusable predicate binding, so there exist incompatible predicates $(W_0, W_1)$ and an adversary $(\cC_\secp, \cU_\secp)$ such that 

\begin{align*}\Pr_{\{\dk_i,\ket{\ck_i},\cCK_i \gets \Gen(1^\secp)\}_{i \in [m]}}&\left[\bigg\|\Pi_{\bdk,\by,W_1}\cU_\secp^{\cCK,\DecZ[\bdk]}\Pi_{\bdk,\by,W_0}\ket{\psi}\bigg\| \geq \frac{1}{\poly(\secp)} : (\ket{\psi},\by) \gets \cC_\secp^{\cCK,\DecZ[\bdk],\DecX[\bdk]}(\ket{\mathbf{\bck}})\right]  \\ & = \frac{1}{\poly(\secp)}. \end{align*}

Observe that for any $\cCK, \bdk, \by,$ and $\ket{\psi}$, 

\begin{align*}
    &\bigg\|\Pi_{\bdk,\by,W_1}\cU_\secp^{\cCK,\DecZ[\bdk]}\Pi_{\bdk,\by,W_0}\ket{\psi}\bigg\| \\ 
    &= \bigg\|\left(\sum_{w_1 \in W_1} \bigotimes_{i: w_{1,i} \neq *}\Pi_{\dk_i,y_i,w_{1,i}} \right) \cU_\secp^{\cCK,\DecZ[\bdk]} \left(\sum_{w_0 \in W_0} \bigotimes_{i: w_{0,i} \neq *}\Pi_{\dk_i,y_i,w_{0,i}} \right) \ket{\psi}\bigg\| \\
    &= \bigg\|\sum_{w_1 \in W_1, w_0 \in W_0} \left(\bigotimes_{i: w_{1,i} \neq *}\Pi_{\dk_i,y_i,w_{1,i}}\right) \cU_\secp^{\cCK,\DecZ[\bdk]} \left(\bigotimes_{i: w_{0,i} \neq *}\Pi_{\dk_i,y_i,w_{0,i}}\right) \ket{\psi} \bigg\| \\ 
    &\leq \sum_{w_1 \in W_1, w_0 \in W_0}\bigg\| \left(\bigotimes_{i: w_{1,i} \neq *}\Pi_{\dk_i,y_i,w_{1,i}}\right) \cU_\secp^{\cCK,\DecZ[\bdk]} \left(\bigotimes_{i: w_{0,i} \neq *}\Pi_{\dk_i,y_i,w_{0,i}}\right) \ket{\psi} \bigg\| \\ 
    &\leq 3^{2m} \max_{w_1,w_0} \bigg\| \left(\bigotimes_{i: w_{1,i} \neq *}\Pi_{\dk_i,y_i,w_{1,i}}\right) \cU_\secp^{\cCK,\DecZ[\bdk]} \left(\bigotimes_{i: w_{0,i} \neq *}\Pi_{\dk_i,y_i,w_{0,i}}\right) \ket{\psi} \bigg\| \\ 
    &\leq 3^{2m} \max_{w_1,w_0} \bigg\| \Pi_{\dk_i,y_i,1-b} \cU_\secp^{\cCK,\DecZ[\bdk]} \Pi_{\dk_i,y_i,b} \ket{\psi} \bigg\|
\end{align*}

for some $(i,b)$ such that $w_{0,i}=b$ and $w_{1,i}=1-b$ , which are always guaranteed to exist by the fact that $W_1$ and $W_0$ are incompatible predicates.

%\takashi{I think it may be better to clarify what are the output of $\widetilde{\cC}_\secp$. I think the first output $\ket{\psi}$ should also contain $i$ (because otherwise $\widetilde{\cU}_\secp$ cannot know $i$) and so this is actually different from that of $\cC_\secp$. The second output should be $y_i$ where $\by=(y_1,...,y_m)$ is that of $\cC_\secp$.}

Now, consider an adversary $(\widetilde{\cC}_\secp, \widetilde{\cU}_\secp)$ defined as follows. 

\begin{itemize}
    \item $\widetilde{\cC}_\secp$ takes as input a single commitment key $\ket{\ck}$, samples $i \gets [m]$, sets $\ket{\ck_i} \coloneqq \ket{\ck}$, samples $\{\dk_j, \ket{\ck_j},\cCK_j \gets \Gen(1^\secp)\}_{j \in [m] \setminus \{i\}}$, and then runs $\cC_\secp$ until it outputs $\ket{\psi}$ and $\by$, responding to $\cCK_i,\DecZ[\dk_i],$ and $\DecX[\dk_i]$ queries by using an external oracle, and $\cCK_j,\DecZ[\dk_j],$ and $\DecX[\dk_j]$ queries for $j \neq i$ internally. Finally, $\widetilde{\cC}_\secp$ outputs $\ket{\widetilde{\psi}} \coloneqq (\ket{\psi},\by,i,\{\dk_j,\cCK_j\}_{j \in [m] \setminus \{i\}})$, and $\widetilde{y} \coloneqq y_i$ where $\by = (y_1,\dots,y_m)$.
    \item $\widetilde{\cU}_\secp$ is the same as $\cU_\secp$, except that $\cCK_i$ and $\DecZ[\dk_i]$ queries are answered by using an external oracle and $\cCK_j$ and $\DecZ[\dk_j]$ queries for $j \neq i$ are answered internally.
\end{itemize}

Then, 

\begin{align*}\Pr_{b \gets \{0,1\},\dk,\ket{\ck},\cCK \gets \Gen(1^\secp)}&\left[\bigg\| \Pi_{\dk,\widetilde{y},1-b} \widetilde{\cU}_\secp^{\cCK,\DecZ[\dk]}\Pi_{\dk,\widetilde{y},b}\ket{\widetilde{\psi}}\bigg\| \geq \frac{1}{3^{2m} \cdot \poly(\secp)} : (\ket{\widetilde{\psi}},\widetilde{y}) \gets \widetilde{\cC}_\secp^{\cCK,\DecZ[\dk],\DecX[\dk]}(\ket{\ck})\right] \\ &\geq \frac{1}{2m \cdot \poly(\secp)},\end{align*} where the $2m$ in the final RHS denominator comes from guessing $b \gets \{0,1\}$ (in the description of the experiment), and $\widetilde{\cC}_\secp$ guessing $i \gets [m]$. Since $3^{2m} \cdot \poly(\secp) \leq 2^{4m}$, and $2m \cdot \poly(\secp) = \poly(\secp)$, this implies that there must exist some $b \in \{0,1\}$ such that 

\begin{align*}\Pr_{\dk,\ket{\ck},\cCK \gets \Gen(1^\secp)}&\left[\bigg\| \Pi_{\dk,\widetilde{y},1-b} \widetilde{\cU}_\secp^{\cCK,\DecZ[\dk]}\Pi_{\dk,\widetilde{y},b}\ket{\widetilde{\psi}}\bigg\| \geq \frac{1}{2^{4m}} : (\ket{\widetilde{\psi}},\widetilde{y}) \gets \widetilde{\cC}_\secp^{\cCK,\DecZ[\dk],\DecX[\dk]}(\ket{\ck})\right] \geq \frac{1}{\poly(\secp)},\end{align*}

which means that the commitment does not satisfy $p \geq 4m$ reusable single-bit binding, a contradiction.


\end{proof}


\subsection{Construction}\label{subsec:SSC-functionality}

Before describing our construction, we introduce some notation.

%A subspace state commitment $\SSC$ consists of two algorithms: a parameter generation algorithm $\SSC.\Gen$ and an (oracle-aided) commitment algorithm $\SSC.\Com$. Before describing these algorithms, we introduce some notation. Let $t = t(\secp), n = n(\secp)$ be some polynomials, which will be parameters of the commitment scheme.

\begin{itemize}
    \item We say that a subspace $S < \bbF_2^n$ is \emph{balanced} if half of its vectors start with 0 and the other half start with 1. Note that $S$ is balanced if and only if at least one of its basis vectors starts with 1. Thus, a random large enough (say $n/2$-dimensional) subspace is balanced with probability $1-\negl(n)$. By default, we will only consider balanced subspaces in what follows.
    \item For an affine subspace $A = S+v$ of $\bbF_2^n$, we write 
    \[\ket{S+v} \coloneqq \frac{1}{\sqrt{|S|}}\sum_{s \in S}\ket{s+v}.\]
    \item Given an affine subspace $S+v$, let $(S+v)^0$ be the set of vectors in $S+v$ that start with 0 and let $(S+v)^1$ be the set of vectors in $S+v$ that start with 1.
    %\item We write $\bS = (S_1,\dots,S_t)$ to refer to a sequence of $t$ subspaces $S_i < \bbF_2^n$, and $\ket{\bS} \coloneqq \ket{\bS_1}\dots\ket{\bS_t}$. Likewise, define $\ket{\bS^0} \coloneqq \ket{S_1^0}\dots\ket{S_t^0}$ and $\ket{\bS^1} \coloneqq \ket{S_1^1}\dots\ket{S_t^1}$.
    %\item $O_\bS$ for $\bS = (S_1,\dots,S_t)$ is the collection of oracles $O_{S_1},\dots,O_{S_t}$ where each $O_{S_i}$ takes as input $v \in \bbF_2^n$ and outputs $\top$ or $\bot$ depending on whether $v \in S_i$ or not.
    %\item $O_\bS^\bot$ for $\bS = (S_1,\dots,S_t)$ is the collection of oracles $O_{S_1}^\bot,\dots,O_{S_t}^\bot$ where each $O_{S_i}^\bot$ takes as input $v \in \bbF_2^n$ and outputs $\top$ or $\bot$ depending on whether $v \in S_i^\bot$ or not.

    

\end{itemize}

We describe our construction of a Pauli Functional Commitment in \cref{fig:PFC-construction}. 

\protocol{Pauli Functional Commitment}{A Pauli Functional Commitment that satisfies \emph{reusable binding}.}{fig:PFC-construction}{

Parameters: Polynomials $t = t(\secp), n = n(\secp) \geq \secp$.\\
Ingredients: Signature token scheme $(\Tok.\Gen,\Tok.\Sign,\Tok.\Verify)$ (\cref{subsec:sig-tokens}).\\

\begin{itemize}
    \item $\Gen(1^\secp)$: Sample uniformly random $n/2$-dimensional balanced affine subspaces $S_1+v_1,\dots,S_t+v_t$ of $\bbF_2^n$ and sample $(\vk,\ket{\sk}) \gets \Tok.\Gen(1^\secp)$. Set \[\dk \coloneqq (S_1,v_1,\dots,S_t,v_t,\vk), \ \ \ \ \ket{\ck} \coloneqq (\ket{S_1+v_1},\dots,\ket{S_t+v_t},\ket{\sk}).\] Define $\cCK$ to take as input $(\sigma,i,s)$ for $i \in [t]$ and $s \in \{0,1\}^n$ and output $\bot$ if $\Tok.\Verify(\vk,0,\sigma) = \bot$, and otherwise output 0 if $s \in S_i^\bot$, and output 1 otherwise.
    \item $\Com_b^{\cCK}(\ket{\ck})$: Parse $\ket{\ck} = (\ket{S_1+v_1}^{\sS_1},\dots,\ket{S_t+v_t}^{\sS_t},\ket{\sk}^{\sK})$. Coherently apply $\Tok.\Sign(1^\secp,0,\cdot)$ from the $\sK$ register to a fresh register $\sG$, which will now hold signatures $\ket{\sigma}$ on the bit 0. Next, repeat the following for each $i \in [t]$.
    \begin{itemize}
        \item Measure the first qubit of register $\sS_i$ in the computational basis. 
        \item If the result is $b$, the state on register $\sS_i$ has collapsed to $\ket{(S_i+v_i)^b}$, and we continue to $i+1$. 
        \item Otherwise, perform a rotation from $\ket{(S_i+v_i)^{1-b}}$ to $\ket{(S_i+v_i)^b}$. This is done by applying the operation $(H^{\otimes n})^{\sS_i}\mathsf{Ph}^{\cCK(\cdot,i,\cdot)}(H^{\otimes n})^{\sS_i}$ to registers $(\sS_i,\sG)$, where $\mathsf{Ph}^{\cCK(\cdot,i,\cdot)}$ is the map $\ket{s}^{\sS_i}\ket{\sigma}^\sG \to (-1)^{\cCK(\sigma,i,s)}\ket{s}^{\sS_i}\ket{\sigma}^\sG$.  
    \end{itemize}
    Next, reverse the $\Tok.\Sign(1^\secp,0,\cdot)$ operation on $(\sK,\sG)$ to recover the state $\ket{\sk}$ on register $\sK$. Finally, sample and output $y \gets \Tok.\Sign(1^\secp,1,\ket{\sk})$, along with the final state on register $\sS \coloneqq (\sS_1,\dots,\sS_t)$.
    \item $\OpenZ(\sB,\sS)$: Measure all registers in the computational basis.
    \item $\OpenX(\sB,\sS)$: Measure all registers in the Hadamard basis.
    \item $\DecZ(\dk,y,z)$: 
    \begin{itemize}
        \item Parse $\dk = (S_1,v_1,\dots,S_t,v_t,\vk)$ and $z = (b,s_1,\dots,s_t)$, where $b \in \{0,1\}$ and $s_i \in \{0,1\}^n$.
        \item Check that $\Tok.\Verify(\vk,1,y) = \top$, and if not output $\bot$.
        \item If for all $i \in [t]$, $s_i \in (S_i + v_i)^b$, output $b$, and otherwise output $\bot$. 
    \end{itemize}
    \item $\DecX(\dk,y,z)$: 
    \begin{itemize}
        \item Parse $\dk = (S_1,v_1,\dots,S_t,v_t,\vk)$ and $z = (b',s_1,\dots,s_t)$, where $b' \in \{0,1\}$ and $s_i \in \{0,1\}^n$.
        \item Check that $\Tok.\Verify(\vk,1,y) = \top$, and if not output $\bot$.
        \item Do the following for each $i \in [t]$: If $s_i \in S_i^\bot$, then define $b_i \coloneqq 0$. If $s_i \oplus (1,0,\dots,0) \in S_i^\bot$, then define $b_i \coloneqq 1$. Otherwise, abort and output $\bot$. That is, $b_i$ is set to 0 if $s_i \in S_i^\bot$ and to 1 if $s_i \in {S_i^0}^\bot \setminus S_i^\bot$. Output $b \coloneqq b' \oplus \bigoplus_{i \in [t]} b_i$. 
    \end{itemize}    
    
    
    
    
    %This is an oracle-aided quantum operation that maps a single qubit register to $1+n\cdot t$ qubits according to $\ket{b} \to \ket{b}\ket{\bS^b}.$ When applied to an arbitrary state, this is the map
    %\[\alpha\ket{0} + \beta\ket{1} \to \alpha\ket{0}\ket{\bS^0} + \beta\ket{1}\ket{\bS^1}.\] Following \cite{10.1145/3357713.3384304}, this map can be efficiently implemented given $\ket{\bS}$ and access to the oracles $O_\bS$ and $O_{\bS}^\bot$.
\end{itemize}
}

%We will also require the following lemma, which we write after introducing more notation.

%\begin{itemize}
    %\item Given $v = (v_1,\dots,v_t) \in (\bbF_2^n)^t$ and $b \in \{0,1\}$, we say that $v \in \bS^b$ if $v_i \in S_i^b$ for all $i \in [t]$, and we say that $v \in {\bS^b}^\bot$ if $v_i \in {S_i^b}^\bot$ for all $i \in [t]$.
    %\item Given $v \in {\bS^0}^\bot$, we define the bit $\mathsf{mask}(v) \coloneqq \bigoplus_{i \in [t]} b_i$, where for each $i \in [t]$, $b_i = 0$ if $v_i \in S_i^\bot$ and $b_i = 1$ if $v_i \notin S_i^\bot$.
%\end{itemize}

%\begin{lemma}\label{lemma:Hadamard-measure}
%Let $\bS = (S_1,\dots,S_t)$ be a sequence of $n/2$-dimensional balanced subspaces of $\bbF_2^n$, and consider any state of the form $\alpha\ket{0}^{\sA}\ket{\bS^0}^\sB + \beta\ket{1}^\sA\ket{\bS^1}^\sB$. Measure the $\sB$ register in the Hadamard basis to obtain a string $v \coloneqq (v_1,\dots,v_t)$, where each $v_i \in \bbF_2^n$. Then it holds that
%\begin{itemize}
    %\item $v \in {\bS^0}^\bot$, and
    %\item the remaining state on register $\sA$ is $\alpha\ket{0} + (-1)^{\mathsf{mask}(v)}\beta\ket{1}$.
%\end{itemize}
%Moreover, checking whether $v \in {\bS^0}^\bot$ and if so, computing $\mathsf{mask}(v)$, can be done just given access to oracles $O_\bS^\bot$.
%\end{lemma}

%\begin{proof}
%\james{TODO: write each $S_i^1$ as $S_i^0 + w_i$ and note that each $v_i \in {S_i^0}^\bot$, and $v_i \cdot w_i$ determines whether $v_i \in S_i^\bot$ or not}
%\end{proof}

\begin{theorem}
The Pauli Functional Commitment described in \cref{fig:PFC-construction} satisfies \emph{correctness} (\cref{def:poc-correctness}).
\end{theorem}

\begin{proof}
We will show correctness assuming that the signature token scheme $\Tok$ is perfectly correct. In reality, it may be statistically correct, but in this case we can still conclude that \cref{fig:PFC-construction} satisfies correctness, which allows for a negligible statistical distance.

We will first show that the map applied by $\Com_b^{\cCK}$ in the case that the measurement of the first qubit of $\sS_i$ is $1-b$ succesfully takes $\ket{(S_i+v_i)^{1-b}} \to \ket{(S_i+v_i)^b}$. Since we are assuming perfect correctness from $\Tok$, it suffices to show that for any balanced affine subspace $\ket{S+v}$, \[H^{\otimes n}\mathsf{Ph}^{O[S^\bot]}H^{\otimes n}\ket{(S+v)^{1-b}} \to \ket{(S+v)^b},\] where $\mathsf{Ph}^{O[S^\bot]}$ is the map $\ket{s} \to (-1)^{O[S^\bot](s)}\ket{s}$, and $O[S^\bot]$ is the oracle that outputs 0 if $s \in S^\bot$ and 1 otherwise. This was actually shown in \cite{STOC:AGKZ20}, but we repeat it here for completeness. 

We will use the facts that $S^1 = S^0 + w$ for some $w$, and that $(S+v)^0 = S^0 + v_0$ and $(S+v)^1 = S^0 + v_1$ for some $v_0,v_1$ such that $v_0 + v_1 = w$. We note that for any $s \in S^\bot$, $s \cdot w = 0$, and for any $s \in {S^0}^\bot \setminus S^\bot$, $s \cdot w = 1$, which will be used in what follows.

\begin{align*}
    H^{\otimes n}&\mathsf{Ph}^{O[S^\bot]}H^{\otimes n}\ket{(S+v)^{1-b}} \\ 
    &= H^{\otimes n} \mathsf{Ph}^{O[S^\bot]}H^{\otimes n}\frac{1}{\sqrt{2^{n/2 - 1}}}\left(\sum_{s \in S^0} \ket{s + v_{1-b}}\right) \\ 
    &= H^{\otimes n}\mathsf{Ph}^{O[S^\bot]}\frac{1}{\sqrt{2^{n/2+1}}}\left(\sum_{s \in {S^0}^\bot}(-1)^{s \cdot v_{1-b}}\ket{s}\right) \\ 
    &= H^{\otimes n}\mathsf{Ph}^{O[S^\bot]}\frac{1}{\sqrt{2^{n/2+1}}}\left(\sum_{s \in S^\bot} (-1)^{s \cdot w + s \cdot v_{b}}\ket{s} + \sum_{s \in {S^0}^\bot \setminus S^\bot} (-1)^{s \cdot w + s \cdot v_{b}} \ket{s}\right) \\ 
    &= H^{\otimes n}\mathsf{Ph}^{O[S^\bot]}\frac{1}{\sqrt{2^{n/2+1}}}\left(\sum_{s \in S^\bot} (-1)^{s \cdot v_{b}}\ket{s} + \sum_{s \in {S^0}^\bot \setminus S^\bot} (-1)^{1 + s \cdot v_{b}} \ket{s}\right) \\ 
    &= H^{\otimes n} \frac{1}{\sqrt{2^{n/2+1}}}\left(\sum_{s \in S^\bot} (-1)^{s \cdot v_b}\ket{s} + \sum_{s \in {S^0}^\bot \setminus S^\bot} (-1)^{s \cdot v_b} \ket{s}\right) \\ 
    &= H^{\otimes n}\frac{1}{\sqrt{2^{n/2+1}}}\left(\sum_{s \in {S^0}^\bot}(-1)^{s \cdot v_b}\ket{s}\right) \\ 
    &= \ket{(S+v)^b}.
\end{align*}

Thus, applying $\Com^{\cCK}$ to a pure state $\ket{\psi} = \alpha_0\ket{0} + \alpha_1\ket{1}$ and commitment key $\ket{\ck}$ produces (up to negligible trace distance) the state \[\ket{\psi_\Com} = \alpha_0\ket{0}\ket{S_1^0}\dots\ket{S_t^0} + \alpha_1\ket{1}\ket{S_1^1}\dots\ket{S_t^1},\] and a signature $y$ on the bit 1.

We continue by arguing that measuring and decoding $\ket{\psi_\Com}$ in either the computational or Hadamard basis produces the same distribution as directly measuring $\ket{\psi}$ in the computational or Hadamard basis. As a mixed state is simply a probability distribution over pure states, this will complete the proof of correctness.

First, it is immediate that measuring $\ket{\psi_\Com}$ in the computational basis produces a bit $b$ with probability $|\alpha_b|^2$ along with vectors $(s_1,\dots,s_t)$ where each $s_i \in (S_i+v_i)^b$. 

Next, note that applying Hadamard to each qubit of $\ket{\psi_\Com}$ except the first results in the state 

\[\alpha_0 \ket{0} \left(\sum_{s \in {S_1^0}^\bot}(-1)^{s \cdot v_{1,0}}\ket{s}\right)\dots\left(\sum_{s \in {S_t^0}^\bot}(-1)^{s \cdot v_{t,0}}\ket{s}\right) + \alpha_1 \ket{1} \left(\sum_{s \in {S_1^0}^\bot}(-1)^{s \cdot v_{1,1}}\ket{s}\right)\dots\left(\sum_{s \in {S_t^0}^\bot}(-1)^{s \cdot v_{t,1}}\ket{s}\right),\] and thus, measuring each of these qubits (except the first) in the Hadamard basis produces vectors $(s_1,\dots,s_t)$ and a single-qubit state \[(-1)^{\bigoplus_{i \in [t]} s_i \cdot v_{i,0}}\alpha_0\ket{0} + (-1)^{\bigoplus_{i \in [t]}s_i \cdot v_{i,1}} \alpha_1\ket{1} = \alpha_0 \ket{0} + (-1)^{s_i \cdot w_i}\alpha_1 \ket{1}.\] So, measuring this qubit in the Hadamard basis is equivalent to measuring $\ket{\psi}$ in the Hadamard basis and masking the result with $\bigoplus_{i \in [t]}s_i \cdot w_i$. Recalling that $s_i \cdot w_i = 0$ if $s_i \in S_i^\bot$ and $s_i \cdot w_i = 1$ if $s_i \in {S_i^0}^\bot \setminus S_i^\bot$ completes the proof of correctness.
\end{proof}



\subsection{Binding}\label{subsec:binding-proof}

%For any subspace $S_i$, let $\Pi_{S_i}^0$ be the projection (in the Hilbert space) onto \emph{non-zero} vectors $v \in S_i$ that start with 0, and let $\Pi_{S_i}^1$ be the projection (in the Hilbert space) onto vectors $v \in S_i$ that start with 1. Then define \[\Pi_\bS^0 \coloneqq \Pi_{S_1}^0 \otimes \dots \otimes \Pi_{S_t}^0, \ \ \ \Pi_\bS^1 \coloneqq \Pi_{S_1}^1 \otimes \dots \otimes \Pi_{S_t}^1.\]

This section is dedicated to proving the following theorem.

\begin{theorem}\label{thm:binding}
Let $p = p(\secp) \geq \secp$ be a polynomial, and assume that $\Tok$ satisfies $3p$ unforgeability. Then the Pauli Functional Commitment described in \cref{fig:PFC-construction}, parameterized by $t = 5p$ and $n = 500t$, satisfies $p$ \emph{reusable single-bit binding} (\cref{def:poc-single-bit-binding}).
\end{theorem}

%For any $p(\secp)$, we will fix $t = t(\secp) < n = n(\secp)$ according to some constraints that will be determined later. 

%We first observe that it suffices to prove the claim with respect to a fixed $b$, say $b=0$. This follows because the distribution over a random affine subspace $S+v$ and over $S+v+e_1$, where $e_1$ is the first standard basis vector, are identical. Thus, any adversary attacking the single-bit binding game for $b$ can be turned into an adversary attacking the single-bit binding game for $1-b$ with the same advantage. \james{TODO: formalize this.} 


%To see this, suppose that we have an adversary $(\cC,\cU)$ attacking the $p$-single-bit-binding game for $b=1$, where here and throughout the proof we will drop the indexing by $\secp$ for notational convenience. Then there exists an adversary $(\widetilde{\cC},\widetilde{\cU})$ that has the same advantage in the $b=0$ game. This follows via the following hybrids.

%\begin{itemize}
    %\item $\cH_0$: The binding game with $(\cC,\cU)$ and $b=1$.
    %\item $\cH_1$: Let $U_{e_1}$ be the unitary acting on $t$ $(n+1)$-qubit registers that flips the first 2 bits of each register, and define $\Pi_{\dk,y,0}'$ and $\Pi_{\dk,y,1}'$ to be the same as $\Pi_{\dk,y,0}'$ and $\Pi_{\dk,y,1}'$ except that they project onto vectors with the same set of bits flipped. Then define $\cC'$ to be the same as $\cC$ except that it applies $U_{e_1}$ at the end to $\ket{\psi}$, and $\cU'$ = $U_{e_1}\cU U_{e_1}$. This is just a re-definition of $\cH_0$.
    %\item $\cH_2$: Sample each affine space as $S_i+v_i+e_1$, where $e_1$ is the first standard basis vector, and let $\widetilde{\cC}$ run $\cC'$ except that it flips the first bit of each  
%\end{itemize}


%Throughout this section, we will consider two-part adversaries $(U_0,U_1)$, where $U_0$ and $U_1$ are \emph{unitary}, and potentially have access to oracles. In the case that $U_0$ and $U_1$ are oracle-aided, then they are technically represented by a sequence of unitaries interleaved with oracle queries. For any such adversary, we define $k$ to be the number of qubits that $U_0$ and $U_1$ act on, and we always assume without loss of generality that $k \geq n$. Finally, when we write projectors $\Pi_\bS^0$ and $\Pi_\bS^1$, which are defined on $n$ qubits, we will implicitly expand them to act on $k \geq n$ qubits by tensoring with the identity, where $k$ is the number of qubits acted on by the adversary. 

The proof of this theorem will be identical for each choice of $b \in \{0,1\}$ in the statement of \cref{def:poc-single-bit-binding}. So, consider any adversary $(\cC,\cU)$ attacking the $p$ reusable single-bit binding game for $b=0$, where we drop the indexing by $\secp$ for notational convenience. We first show that it suffices to prove the following claim, in which $\cU$ no longer has oracle access to $\cCK$. We will also switch to working with the norm squared for convenience throughout the rest of this proof.

\begin{claim}\label{claim:no-com-oracle}
For any $(\cC,\cU)$ where $\cC$ and $\cU$ each make $\poly(\secp)$ many oracle queries, it holds that 
\[\Pr_{\dk,\ket{\ck},\cCK \gets \Gen(1^\secp)}\left[\bigg\|\Pi_{\dk,y,1}\cU^{\DecZ[\dk]}\Pi_{\dk,y,0}\ket{\psi}\bigg\|^2 \geq \frac{1}{2^{2p+1}} : (\ket{\psi},y) \gets \cC^{\cCK,\DecZ[\dk],\DecX[\dk]}(\ket{\ck})\right] = \negl(\secp).\]
\end{claim}

\begin{lemma}
\cref{claim:no-com-oracle} implies \cref{thm:binding}.
\end{lemma}

\begin{proof}

First, we-restate \cref{thm:binding} with respect to the norm squared. That is, for any $(\cC,\cU)$ with $\poly(\secp)$ many oracle queries, it holds that 

\[\Pr_{\dk,\ket{\ck},\cCK \gets \Gen(1^\secp)}\left[\bigg\|\Pi_{\dk,y,1}\cU^{\cCK,\DecZ[\dk]}\Pi_{\dk,y,0}\ket{\psi}\bigg\|^2 \geq \frac{1}{2^{2p}} : (\ket{\psi},y) \gets \cC^{\cCK,\DecZ[\dk],\DecX[\dk]}(\ket{\ck})\right] = \negl(\secp).\]

To show that \cref{claim:no-com-oracle} implies the above statement, we define the oracle $\cO_\bot$ to always map $(\sigma,i,s) \to \bot$, and then argue that 

\[\E_{\substack{\dk,\ket{\ck},\cCK \gets \Gen(1^\secp) \\ (\ket{\psi},y) \gets \cC^{\cCK,\DecZ[\dk],\DecX[\dk]}(\ket{\ck})}}\left[\bigg\| \Pi_{\dk,y,1}\cU^{\cCK,\DecZ[\dk]}\Pi_{\dk,y,0}\ket{\psi} \bigg\|^2 - \bigg\| \Pi_{\dk,y,1}\cU^{\cO_\bot,\DecZ[\dk]}\Pi_{\dk,y,0}\ket{\psi} \bigg\|^2 \right] \leq \frac{\poly(\secp)}{2^{3p}}.\]

This follows from a standard hybrid argument, by reduction to the $3p$ unforgeability of the signature token scheme. Consider replacing each $\cCK$ oracle query with a $\cO_\bot$ oracle query one by one, starting with the last query. That is, we define hybrid $\cH_0$ to be \[\E_{\substack{\dk,\ket{\ck},\cCK \gets \Gen(1^\secp) \\ (\ket{\psi},y) \gets \cC^{\cCK,\DecZ[\dk],\DecX[\dk]}(\ket{\ck})}}\left[\bigg\| \Pi_{\dk,y,1}\cU^{\cCK,\DecZ[\dk]}\Pi_{\dk,y,0}\ket{\psi} \bigg\|^2 \right],\] and in hybrid $\cH_i$, we switch the $i$'th from the last query from being answered by $\cCK$ to being answered by $\cO_\bot$. Now, fix any $i$, and consider measuring the query register of $\cU$'s $i$'th from last query to obtain classical strings $(\sigma,i,s)$. Then since $\Pi_{\dk,y,0}$ is the zero projector when $y$ is not a valid signature on 1, and $\cCK$ outputs $\bot$ whenever $\sigma$ is not a valid signature on 1, we have that

\[\E[\cH_{i-1} - \cH_i] \leq \Pr[\Tok(\vk,1,y) = 1 \wedge \Tok(\vk,0,\sigma) = 1] \leq \frac{1}{2^{3p}},\] by the $3p$ unforgeability of the signature token scheme. Since there are $\poly(\secp)$ many hybrids, this completes the hybrid argument.

Finally, it follows by Markov that 

\begin{align*}\Pr_{\substack{\dk,\ket{\ck},\cCK \gets \Gen(1^\secp) \\ (\ket{\psi},y) \gets \cC^{\cCK,\DecZ[\dk],\DecX[\dk]}(\ket{\ck})}}&\left[\bigg\| \Pi_{\dk,y,1}\cU^{\cCK,\DecZ[\dk]}\Pi_{\dk,y,0}\ket{\psi} \bigg\|^2 - \bigg\| \Pi_{\dk,y,1}\cU^{\cO_\bot,\DecZ[\dk]}\Pi_{\dk,y,0}\ket{\psi} \bigg\|^2 \geq \frac{1}{2^{2p+1}}\right]\\ &\leq \frac{\poly(\secp)}{2^{p-1}} = \negl(\secp),
\end{align*} which completes the proof.

\end{proof}

Now, we introduce some more notation.

\begin{itemize}
    \item Given polynomials $t = t(\secp), k = k(\secp)$, and $n = n(\secp)$, we write $\ASGen(1^\secp,t,k,n)$ to refer to the procedure that samples $t$ uniformly random balanced affine subspaces of $\bbF_2^n$ of dimension $k$.
    \item Given a sequence of affine subspaces $(A_1 = S_1+v_1,\dots,A_t = S_t+v_t)$, we define $\bA \coloneqq (A_1,\dots,A_t)$, $\ket{\bA} \coloneqq \ket{A_1},\dots,\ket{A_t}$, and for $b \in \{0,1\}$, $\ket{\bA^b} \coloneqq \ket{A_1^b},\dots,\ket{A_t^b}$. 
    \item For a sequence of affine subspaces $\bA = (S_1+v_1,\dots,S_t+v_t)$, let $O[\bA]$ be the collection of oracles $O[A_1],\dots,O[A_t]$, where each $O[A_i]$ checks for membership in $A_i$, and let $O[\bA^\bot]$ be the collection of oracles $O[S_1^\bot],\dots,O[S_t^\bot]$, where each $O[S_i^\bot]$ checks for membership in $S_i^\bot$.
    \item For a sequence of affine subspaces $\bA$ and $b \in \{0,1\}$, define the projector $\Pi[\bA^b] \coloneqq \Pi[A_1^b] \otimes \dots \otimes \Pi[A_t^b]$, where each $\Pi[A_i^b]$ is the projection onto vectors $s \in A_i^b$.
\end{itemize}


We will use this notation to re-define the game in \cref{claim:no-com-oracle}, and show that it suffices to prove the following claim.


%Now, consider any adversary $(\cC,\cU)$ attacking the $p$-single-bit-binding of the commitment scheme, where we drop the indexing by $\secp$ for notational convenience. We can always consider a purification of $\cC$, which we denote by a unitary $U_\Com$. Re-naming $\cU$ to $U_\Open$ and making use of the just-introduced notation, we see that the following claim suffices to prove \cref{thm:binding}.


\begin{claim}\label{claim:A-oracle}
For any two unitaries $(U_\Com,U_\Open)$, where $U_\Com$ and $U_\Open$ each make $\poly(\secp)$ many oracle queries, it holds that

\[\Pr_{\bA \gets \ASGen(1^\secp,t,n/2,n)}\left[\bigg\|\Pi[\bA^1]U_\Open^{O[\bA]}\Pi[\bA^0]\ket{\psi}\bigg\|^2 \geq \frac{1}{2^{2p+1}} : \ket{\psi} \coloneqq U_\Com^{O[\bA],O[\bA^\bot]}(\ket{\bA})\right] = \negl(\secp).\]
\end{claim}

\begin{lemma}
\cref{claim:A-oracle} implies \cref{claim:no-com-oracle}.
\end{lemma}

\begin{proof}
First, we note that re-defining $\Pi_{\dk,y,b}$ in the statement of \cref{claim:no-com-oracle} to ignore $y$ and only check for membership in the affine subspaces $\{(S_i+v_i)^b\}_{i \in [t]}$ only potentially increases the squared norm of the resulting vector. This means that we can also ignore the $y$ output by $\cC$. Next, we observe that it is straightforward to simulate the $\DecZ[\dk]$ oracle with $O[\bA]$, where $\bA$ are the affine subspaces defined by $\dk$, and also to simulate the $\DecX[\dk]$ oracle with $O[\bA^\bot]$. Finally, we can purify any operation $\cC$ to consider a unitary $U_\Com$ that outputs $\ket{\psi}$.
\end{proof}



Our next step is to remove $U_\Open$'s oracle access to $O[\bA]$. We will show that it suffices to prove the following. 

%First, consider altering the $\SSC.\Gen(1^\secp,t,n)$ algorithm to output a sequence of balanced subspaces $S_i$ of dimension $2n/3$ rather than $n/2$. We denote this sampling algorithm by $\SSC.\Gen^{2/3}(1^\secp,t,n)$. 

%\begin{claim}\label{claim:remove-oracle}
%Consider any two-part adversary $(U_0,U_1)$, where $U_0$ makes $\poly(\secp)$ many oracle queries. Then it holds that

%\[\Pr_{\bS \gets \SSC.\Gen^{2/3}(1^\secp,t,n)}\left[\bra{\psi}\Pi_\bS^0U_1^\dagger\Pi_\bS^1U_1\Pi_\bS^0\ket{\psi} \geq \frac{1}{2^{p(\secp)}} : \ket{\psi} \coloneqq U_0^{O_\bS,O^\bot_\bS}(\ket{\bS})\right] = \negl(\secp).\]
%\end{claim}


\begin{claim}\label{claim:remove-oracle}
For any two unitaries $(U_\Com,U_\Open)$, where $U_\Com$ makes $\poly(\secp)$ many oracle queries, it holds that

\[\Pr_{\bA \gets \ASGen(1^\secp,t,n/2,3n/4)}\left[\bigg\|\Pi[\bA^1]U_\Open\Pi[\bA^0]\ket{\psi}\bigg\|^2 \geq \frac{1}{2^{2p+2}} : \ket{\psi} \coloneqq U_\Com^{O[\bA],O[\bA^\bot]}(\ket{\bA})\right] = \negl(\secp).\]
\end{claim}

Notice that $\ASGen$ is now sampling affine subspaces of a $3n/4$-dimensional space. 


\begin{lemma}
\cref{claim:remove-oracle} implies \cref{claim:A-oracle}.
\end{lemma}

\begin{proof}

Given $n/2$-dimensional affine subspaces $\bA = (A_1,\dots,A_t)$, consider sampling uniformly random $3n/4$-dimensional subspaces $\bT = (T_1,\dots,T_t)$ such that each $A_i \subset T_i$. We will denote this procedure by $\bT \gets \mathsf{Super}(3n/4,\bA)$. Then, define $O[\bT \setminus \{0^n\}]$ to be the collection of oracles $O[T_1 \setminus \{0^n\}],\dots,O[T_t \setminus \{0^n\}]$, where each $O[T_i \setminus \{0^n\}]$ checks for membership in the set $T_i \setminus \{0^n\}$.

Now, we will show via a standard hybrid argument that 

\[\E_{\substack{\bA \gets \ASGen(1^\secp,t,n/2,n) \\ \bT \gets \mathsf{Super}(3n/4,\bA) \\ \ket{\psi} \coloneqq U_\Com^{O[\bA],O[\bA^\bot]}(\ket{\bA})}}\left[\bigg\| \Pi[\bA^1]U_\Open^{O[\bA]}\Pi[\bA^0]\ket{\psi}\bigg\|^2 - \bigg\| \Pi[\bA^1]U_\Open^{O[\bT \setminus \{0^n\}]}\Pi[\bA^0]\ket{\psi}\bigg\|^2\right] \leq \frac{\poly(\secp)}{2^{n/4}}.\]

Consider replacing each $O[\bA]$ oracle query with a $O[\bT \setminus \{0^n\}]$ oracle query one by one, starting with the last query. That is, we define hybrid $\cH_0$ to be \[\E_{\substack{\bA \gets \ASGen(1^\secp,t,n/2,n) \\ \bT \gets \mathsf{Super}(3n/4,\bA) \\ \ket{\psi} \coloneqq U_\Com^{O[\bA],O[\bA^\bot]}(\ket{\bA})}}\left[\bigg\| \Pi[\bA^1]U_\Open^{O[\bA]}\Pi[\bA^0]\ket{\psi}\bigg\|^2\right],\] and in hybrid $\cH_i$, we switch the $i$'th from the last query from being answered by $O[\bA]$ to being answered by $O[\bT \setminus \{0^n\}]$. Then, for any $i$, let $p(i) \in [t]$ be the index of the oracle queried by $U_\Open$ on its $i$'th to last query. By \cref{claim:max-prob}, we have that \[\E[\cH_{i-1} - \cH_i] \leq \max_{s}\Pr_{T_{p(i)}}[s \in T_{p(i)} \setminus S_{p(i)} \setminus \{0^n\}] \leq \frac{1}{2^{n/4}}.\]

Since there are $\poly(\secp)$ many hybrids, this completes the hybrid argument. Now, it follows by Markov that 

\begin{align*}\Pr_{\substack{\bA \gets \ASGen(1^\secp,t,n/2,n) \\ \bT \gets \mathsf{Super}(3n/4,\bA) \\ \ket{\psi} \coloneqq U_\Com^{O[\bA],O[\bA^\bot]}(\ket{\bA})}}&\left[\bigg\| \Pi[\bA^1]U_\Open^{O[\bA]}\Pi[\bA^0]\ket{\psi}\bigg\|^2 - \bigg\| \Pi[\bA^1]U_\Open^{O[\bT \setminus \{0^n\}]}\Pi[\bA^0]\ket{\psi}\bigg\|^2 \geq \frac{1}{2^{2p+2}}\right]\\ &\leq \frac{\poly(\secp)2^{2p+2}}{2^{n/4}} = \negl(\secp),\end{align*} since $n \geq 9p$. Finally, this implies the lemma, since we can imagine fixing $\bT$ as a public sequence of ambient subspaces of dimension $3n/4$ and sampling $\bA$ as a random sequence of affine subspaces of $\bT$.



%Suppose that there exists $(U_\Com, U_\Open)$ that violates \cref{claim:binding}. Given $\bS = (S_1,\dots,S_t)$, consider sampling uniformly random $3n/4$-dimensional superspaces $\bS' = (S_1',\dots,S_t')$ and giving $U_\Open$ oracle access to $O[\bS']$ rather than $O[\bS]$. Recall that $O[\bS]$ actually represents the collection of oracles $O[S_1],\dots,O[S_t]$, so each of $U_\Open$'s oracle queries is made specifically to one of the oracles $O[S_i]$. 

%We claim that for any fixed $\bS$ and $\ket{\psi}$,

%\[\E_{\bS' > \bS}\left[\TD\left(U_\Open^{O[\bS]}\ket{\psi},U_\Open^{O[\bS']}\ket{\psi}\right)\right] \leq \frac{q}{2^{n/4}},\] where $q = \poly(\secp)$ is the number of the oracle queries that $U_\Open$ makes, and the expectation is over sampling $\bS'$ as a uniformly random sequence of $3n/4$-dimensional superspaces of $(S_1,\dots,S_t)$. To see this, we consider a sequence of hybrid states, using the following notation.

%\begin{itemize}
    %\item Let $\ket{\psi_0} = U_\Open^{O[\bS]}\ket{\psi}$.
    %\item Let $\ket{\psi_q} = U_\Open^{O[\bS']}\ket{\psi}$.
    %\item Let $\ket{\psi_j}$ be the state that results from running $U_\Open$ on $\ket{\psi}$, answering the first $q-j$ oracle queries with $O[\bS]$ and the final $j$ oracle queries with $O[\bS']$.
    %\item Let $\ket{\widetilde{\psi}_j}$ be the state right before the $(q-j+1)$'th oracle query in the $(j-1)$'th hybrid is answered. 
    %\item Let $\ket{\widetilde{\psi}_j'}$ be the component of $\ket{\widetilde{\psi}_j}$ on vectors in $S'_i \setminus S_i$, where $i$ is the index of the oracle that $U_\Open$ queries on its $j$'th query. 
%\end{itemize}

%Then we have that for any $j \in [q]$,

%\[\E_{\bS' > \bS}\left[\TD\left(\ket{\psi_{j-1}},\ket{\psi_j}\right)\right] = \E_{\bS' > \bS}\left[\|\ket{\widetilde{\psi}_j'}\|^2\right] \leq \max_{s \notin S_i}\Pr_{S'_i}[s \in S'_i] \leq \frac{1}{2^{n/4}},\] which establishes the trace distance claim above. Thus, it holds that 

%\[\E_{\bS' > \bS}\left[\bigg|\bigg\|\Pi[\bS^1]U_\Open^{O[\bS]}\Pi[\bS^0]\ket{\psi}\bigg\|^2 - \bigg\|\Pi[\bS^1]U_\Open^{O[\bS']}\Pi[\bS^0]\ket{\psi}\bigg\|^2 \bigg|\right] \leq \frac{q}{2^{n/4}},\] so by Markov,

%\[\Pr\left[\bigg\|\Pi[\bS^1]U_\Open^{O[\bS']}\Pi[\bS^0]\ket{\psi}\bigg\|^2 \leq \bigg\|\Pi[\bS^1]U_\Open^{O[\bS]}\Pi[\bS^0]\ket{\psi}\bigg\|^2 - \frac{\sqrt{q}}{2^{n/8}}\right] \leq \frac{\sqrt{q}}{2^{n/8}}.\]

%Now, since $q = \poly(\secp), n \geq \secp$, and $n \geq 9 \cdot p$, this implies that \[\Pr_{\bS \gets \SSGen(1^\secp,t,n/2,n), \bS' > \bS}\left[\bigg\|\Pi[\bS^1]U_\Open^{O[\bS']}\Pi[\bS^0]\ket{\psi}\bigg\|^2 \geq \frac{1}{2^{p(\secp)+1}} : \ket{\psi} \coloneqq U_\Com^{O[\bS],O[\bS^\bot]}(\ket{\bS})\right] = 1/\poly(\secp).\]

%Thus, $(U_\Com,U_\Open)$ violates \cref{claim:remove-oracle}, since we can imagine fixing $\bS'$ as a sequence of ambient spaces of dimension $3n/4$, and sampling $\bS$ as a sequence of $n/2$-dimensional subspaces. In this scenario, $U_\Open$ no longer requires oracle access since $\bS'$ is fixed and public. This completes the proof.

%\james{TODO: This reduction holds because $U_\Open$ won't be able to tell whether it gets oracle access to $O[\bS]$ or $O[\bS']$ where $\bS'$ are sampled as $3n/4$-dimensional superspaces of $\bS$. Then, we can just give $\bS'$ to $(U_\Com,U_\Open)$ in the clear.}

\end{proof}

Next, we perform a worst-case to average-case reduction over the sampling of $\bA$ and thus show that it suffices to prove the following.

\begin{claim}\label{claim:worst-case}
There do not exist two unitaries $(U_\Com,U_\Open)$, where $U_\Com$ makes $\poly(\secp)$ many oracle queries, such that for all $\bA \in \ASGen(1^\secp,t,n/2,3n/4)$ it holds that \[\bigg\|\Pi[\bA^1]U_\Open\Pi[\bA^0]\ket{\psi_\bA}\bigg\|^2 \geq \frac{1}{2^{2p+3}},\] where $\ket{\psi_{\bA}} \coloneqq U_\Com^{O[\bA],O[\bA^\bot]}(\ket{\bA})$.
\end{claim}

\begin{lemma}
\cref{claim:worst-case} implies \cref{claim:remove-oracle}.
\end{lemma}

\begin{proof}

Suppose that there exists $(U_\Com,U_\Open)$ that violates \cref{claim:remove-oracle}. We define an adversary $(\widetilde{\cC},\widetilde{U}_\Open)$ as follows.

\begin{itemize}
    \item $\widetilde{\cC}$ takes $\ket{\bA}$ as input. For each $i \in [t]$, it samples a uniformly random change of basis $B_i$ of $\bbF_2^{3n/4}$ and defines $\bB \coloneqq (B_1,\dots,B_t)$. Define the unitary $U_\bB$ acting on $t \cdot n$ qubits to map $\ket{s_1}\dots\ket{s_t} \to \ket{B_1(s_1)}\dots\ket{B_t(s_t)}$.
    \item Run $U_\Com$ on $\ket{\bB(\bA)} = \ket{B_1(A_1)}\dots\ket{B_t(A_t)}$. Answer each of $U_\Com$'s oracle queries with $U_\bB O[\bA] U_\bB^\dagger$ or $U_\bB O[\bA^\bot] U_\bB^\dagger$, where $U_\bB$ acts on the query register.
    \item Let $\ket{\psi}$ be $U_\Com$'s output, and output $\ket{\widetilde{\psi}} \coloneqq (U_\bB^\dagger\ket{\psi},\bB)$, where register $\sB$ holds $\bB$, which is the classical description of the sequence of change of bases.
    \item $\widetilde{U}_\Open$ is defined to be $U_{\mathsf{CoB}^{-1}} U_\Open U_{\mathsf{CoB}}$, where \[U_{\mathsf{CoB}} \coloneqq \frac{1}{\#\bB}\sum_{\bB}U_\bB \otimes \ket{\bB}\bra{\bB}^\sB, \ \ \ \text{and} \ \ \ U_{\mathsf{CoB}^{-1}} \coloneqq \frac{1}{\#\bB}\sum_{\bB}U^\dagger_\bB \otimes \ket{\bB}\bra{\bB}^\sB,\] where $\#\bB$ counts the total number of sequences of change of bases $\bB$.
\end{itemize}

Then since for any fixed $\bA$ and uniformly random $\bB$, it holds that $\bB(\bA)$ is a uniformly random sequence of affine subspaces, we see that for any $\bA \in \ASGen(1^\secp,t,n/2,3n/4)$,

\begin{align*}
&\Pr\left[\bigg\|\Pi[\bA^1]\widetilde{U}_\Open\Pi[\bA^0]\ket{\widetilde{\psi}}\bigg\|^2 \geq \frac{1}{2^{2p+2}} : \ket{\widetilde{\psi}} \gets \widetilde{\cC}^{O[\bA],O[\bA^\bot]}(\ket{\bA})\right] \\
&= \Pr_{\bB(\bA) \gets \ASGen(1^\secp,t,n/2,3n/4)}\left[\bigg\|\Pi[{\bB(\bA)}^1]U_\Open\Pi[{\bB(\bA)}^0]\ket{\psi}\bigg\|^2 \geq \frac{1}{2^{2p+2}} : \ket{\psi} \gets U_\Com^{O[\bB(\bA)],O[{\bB(\bA)}^\bot]}(\ket{\bB(\bA)})\right]\\ &= \nonnegl(\secp).\end{align*}

Now, define $\ket{\widetilde{\psi}_\bB}$ to be the output of $\widetilde{\cC}$ conditioned on sampling $\bB$. Then define $\widetilde{U}_\Com$ to be a purification of $\cC$. It holds that for any fixed $\bA \in \ASGen(1^\secp,t,n/2,3n/4)$ and $\ket{\widetilde{\psi}} \coloneqq \widetilde{U}_\Com^{O[\bA],O[\bA^\bot]}(\ket{\bA})$,

\begin{align*}
    \bigg\| \Pi[\bA^1]\widetilde{U}_\Open \Pi[\bA^0]\ket{\widetilde{\psi}}\bigg\|^2 = \frac{1}{\#\bB}\sum_{\bB}\bigg\| \Pi[\bA^1]\widetilde{U}_\Open\Pi[\bA^0]\ket{\widetilde{\psi}_\bB}\bigg\|^2 \geq \nonnegl(\secp) \cdot \frac{1}{2^{2p+2}} \geq \frac{1}{2^{2p+3}},
\end{align*}

which completes the proof.
\end{proof}

For the rest of this proof, we will fix an arbitrary unitary $U_\Open$. Given a sequence of affine subspaces $\bA$, we define

\[\Pi[\bA]_0 \coloneqq \Pi[\bA^0], \ \ \, \Pi[\bA]_1 \coloneqq U_\Open^\dagger \Pi[\bA^1] U_\Open.\] 

Next, consider the (not necessarily unique) singular value decomposition

\[\Pi[\bA]_1\Pi[\bA]_0 = U\Sigma V,\]

where $U$ and $V$ are unitary and $\Sigma$ is a diagonal matrix of singular values $\{s_i\}_i$. The $i$'th singular value $s_i$ on the diagonal is associated with the $i$'th row $\bra{\phi_i}$ of $V$ (a right singular vector) and the $i$'th column $\ket{\tau_i}$ of $U$ (a left singular vector). For any $\epsilon \in (0,1)$, we define \[\Thr[\bA]_\epsilon\] to be the projector onto the subspace spanned by right singular vectors $\bra{\phi_i}$ of $\Pi[\bA]_1\Pi[\bA]_0$ with singular value $s_i$ such that $s_i^2 \geq \epsilon$. Note that $\mathsf{Im}(\Thr[\bA]_\epsilon)$ is a subspace of $\mathsf{Im}(\Pi[\bA]_0)$. We will also use the following key property of $\Thr[\bA]_\epsilon$. 


\begin{fact}\label{fact:thr}
For any $\ket{\psi}$, \[\big\|\Pi[\bA]_1\Pi[\bA]_0\ket{\psi}\big\|^2 - \epsilon \leq \big\|\Thr[\bA]_\epsilon\ket{\psi}\big\|^2 \leq \frac{\big\|\Pi[\bA]_1\Pi[\bA]_0\ket{\psi}\big\|^2}{\epsilon}.\]
\end{fact}


%\begin{enumerate}
    %\item For any $\ket{\psi}$, \[\big\|\Thr[\bA]_\epsilon\ket{\psi}\big\|^2 \geq \big\|\Pi[\bA]_1\Pi[\bA]_0\ket{\psi}\big\|^2 - \epsilon.\] 
    %\item For any $\ket{\psi}$,
    %\[\big\| \Pi[\bA]_1\Pi[\bA]_0\ket{\psi}\big\|^2 \geq \epsilon \cdot \big\| \Thr[\bA]_\epsilon\ket{\psi}\big\|^2.\]
%\end{enumerate}

\begin{proof}

The left inequality follows because
    
    \begin{align*}
        \big\|\Pi[\bA]_1\Pi[\bA]_0\ket{\psi}\big\|^2 &= \big\|\Pi[\bA]_1\Thr[\bA]_\epsilon \Pi[\bA]_0\ket{\psi} + \Pi[\bA]_1(\bbI - \Thr[\bA]_\epsilon) \Pi[\bA]_0\ket{\psi}\big\|^2 \\ &= \big\|\Pi[\bA]_1\Thr[\bA]_\epsilon \Pi[\bA]_0\ket{\psi}\big\|^2 + \big\|\Pi[\bA]_1(\bbI - \Thr[\bA]_\epsilon) \Pi[\bA]_0\ket{\psi}\big\|^2 \\
        &\leq \big\|\Pi[\bA]_1\Thr[\bA]_\epsilon \Pi[\bA]_0\ket{\psi}\big\|^2 + \epsilon \\
        &\leq \big\|\Thr[\bA]_\epsilon\ket{\psi}\big\|^2 +\epsilon,
    \end{align*}
    
where the second equality is due to the fact that for any $\ket{\psi} \in \mathsf{Im}(\Pi[\bA]_0)$, \[\Pi[\bA]_1\Thr[\bA]_\epsilon\ket{\psi} \in \mathsf{Span}\left(\{\ket{\tau_i}\}_{i: s_i^2 \geq \epsilon}\right), \ \ \ \text{and} \ \ \ \Pi[\bA]_1(\bbI-\Thr[\bA]_\epsilon)\ket{\psi} \in \mathsf{Span}\left(\{\ket{\tau_i}\}_{i: s_i^2 < \epsilon}\right),\] and thus the two vectors are orthogonal.
    
The right inequality follows because \[\big\|\Pi[\bA]_1 \Pi[\bA]_0\ket{\psi}\big\|^2 \geq \big\|\Pi[\bA]_1\Thr[\bA]_\epsilon \Pi[\bA]_0\ket{\psi}\big\|^2 \geq \epsilon \cdot \big\|\Thr[\bA]_\epsilon \Pi[\bA]_0\ket{\psi}\big\|^2 = \epsilon \cdot \big\| \Thr[\bA]_\epsilon\ket{\psi}\big\|^2.\]

\end{proof} 

%\takashi{Is $\Pi[\bA]_0$ redundant?}
%\ryo{Even we remove $\Pi[\bA]_0$, the inequality does not seem to be correct. Bounded by $\big\|\Pi[\bA]_1\Pi[\bA]_0\ket{\psi}\big\|^2$ or $\big\|\Pi[\bA]_1\Thr[\bA]_\epsilon \ket{\psi}\big\|$?}

Now, we will show via amplitude amplification that it suffices to prove the following claim.

\begin{claim}\label{claim:jor}
Let $\epsilon = 1/2^{3p}$. There do not exist two unitaries $(U_\Com,U_\Open)$ where $U_\Com$ makes at most $2^{51t}$ oracle queries, such that for all $\bA \in \ASGen(1^\secp,t,n/2,3n/4)$ it holds that
\[\bigg\|\Thr[\bA]_\epsilon\ket{\psi_\bA}\bigg\|^2 \geq 1-\frac{1}{2^{4t}},\] where $\ket{\psi_\bA} \coloneqq U_\Com^{O[\bA],O[\bA^\bot]}(\ket{\bA})$.
\end{claim}

\begin{lemma}
\cref{claim:jor} implies \cref{claim:worst-case}.
\end{lemma}

\begin{proof}

First, we will introduce the following notation. For any binary projective measurement $(\Pi, \bbI - \Pi)$, we define $U_\Pi$ to be a unitary that maps $\ket{\phi} \to - \ket{\phi}$ for any $\ket{\phi} \in \mathsf{Im}(\Pi)$ and acts as the identity on all $\ket{\phi}$ orthogonal to $\Pi$.

We will use the following two imported theorems.

\begin{importedtheorem}[Approximate singular value threshold projection, \cite{STOC:GSLW19} Theorem 31]\label{thm:alternating-projectors}
There exists an oracle-aided algorithm $\mathsf{Threshold}$ that outputs one bit, is parameterized by $(\beta,\delta,\gamma)$, and has the following properties. Consider any two binary projective measurements $(\Pi_0, \bbI - \Pi_0)$ and $(\Pi_1, \bbI - \Pi_1)$. Then for any right singular vector $\ket{\phi}$ of $\Pi_1\Pi_0$ with singular value $s$,
\begin{itemize}
    \item if $s^2 \geq \beta$, then $\Pr\left[1 \gets \mathsf{Threshold}^{U_{\Pi_0},U_{\Pi_1}}_{\beta,\delta,\gamma}(\ket{\phi})\right] \geq 1-\gamma$,
    \item and if $s^2 \leq \beta-\delta$, then $\Pr\left[1 \gets \mathsf{Threshold}^{U_{\Pi_0},U_{\Pi_1}}_{\beta,\delta,\gamma}(\ket{\phi}) \right] \leq \gamma$.
\end{itemize}
Moreover, $\mathsf{Threshold}^{U_{\Pi_0},U_{\Pi_1}}_{\beta,\delta,\gamma}$ makes $O(\log(1/\gamma)/\delta)$ oracle queries.
\end{importedtheorem}

%We will also make use of the following imported theorem.

\begin{importedtheorem}[Fixed-point amplitude amplification, \cite{STOC:GSLW19} Theorem 27]\label{thm:quantum-search}
There exists an oracle-aided unitary $\mathsf{Amplify}$ that is parameterized by $(\eta,\zeta)$, and has the following properties. Let $\ket{\psi}$ and $\ket{\psi_G}$ be normalized states and $\Pi$ be a projector such that $\Pi\ket{\psi} = \nu\ket{\psi_G}$, where $\nu \geq \eta$. Then $\ket{\widetilde{\psi}_G} \coloneqq \mathsf{Amplify}_{\eta,\zeta}^{U_{\ket{\psi}\bra{\psi}},U_\Pi}(\ket{\psi})$ is such that $\|\ket{\psi_G} - \ket{\widetilde{\psi}_G}\| \leq \zeta$. Moreover, $\mathsf{Amplify}_{\eta,\zeta}^{U_{\ket{\psi}\bra{\psi}},U_\Pi}(\ket{\psi})$ makes $O(\log(1/\zeta)/\eta)$ oracle queries.
\end{importedtheorem}


Now, consider any $(U_\Com, U_\Open)$ that violates \cref{claim:worst-case}, and fix any $\bA \in \ASGen(1^\secp,t,n/2,3n/4)$. Also fix the parameters \[\eta = \frac{1}{2^t}, \ \ \zeta = \frac{1}{2^{12t}}, \ \ \gamma = \frac{1}{2^{24t}}, \ \ \ell = 24t.\]


Define \[\ket{\psi_{\bA^0}} \coloneqq \frac{\Pi[\bA]_0\ket{\psi_\bA}}{\|\Pi[\bA]_0\ket{\psi_\bA}\|}, \ \ \ \ket{\widetilde{\psi}_{\bA^0}} \coloneqq \Amplify_{\eta,\zeta}^{U_{\ket{\psi_\bA}\bra{\psi_\bA}},U_{\Pi[\bA]_0}}(\ket{\psi_\bA}),\] and write \[\ket{\widetilde{\psi}_{\bA^0}} \coloneqq \ket{\psi_{\bA^0}} + \ket{\psi_{\bA^0}^{\err}}.\]

For $i \in [2^\ell]$, define \[\widetilde{\Thr}[\bA]_i \coloneqq \left(\mathsf{U}\text{-}\mathsf{Threshold}_{\epsilon+i/2^{2\ell},1/2^{2\ell},\gamma}^{\Pi[\bA]_0,\Pi[\bA]_1}\right)^\dagger \ket{1}\bra{1} \left(\mathsf{U}\text{-}\mathsf{Threshold}_{\epsilon+i/2^{2\ell},1/2^{2\ell},\gamma}^{\Pi[\bA]_0,\Pi[\bA]_1}\right),\] where $\mathsf{U}\text{-}\mathsf{Threshold}_{\epsilon+i/2^{2\ell},1/2^{2\ell},\gamma}^{\Pi[\bA]_0,\Pi[\bA]_1}$ is the purification of $\mathsf{Threshold}_{\epsilon+i/2^{2\ell},1/2^{2\ell},\gamma}^{\Pi[\bA]_0,\Pi[\bA]_1}$. 


Define \[\ket{\psi_{\Thr,i}} \coloneqq \frac{\widetilde{\Thr}[\bA]_i\ket{\widetilde{\psi}_{\bA^0}}}{\| \widetilde{\Thr}[\bA]_i\ket{\widetilde{\psi}_{\bA^0}}\|}, \ \ \ \ket{\widetilde{\psi}_{\Thr,i}} \coloneqq \Amplify_{\eta,\zeta}^{U_{\ket{\widetilde{\psi}_{\bA^0}}\bra{\widetilde{\psi}_{\bA^0}}},U_{\widetilde{\Thr}[\bA]_i}}(\ket{\widetilde{\psi}_{\bA^0}}),\]

and write \[\ket{\widetilde{\psi}_{\Thr,i}} \coloneqq \ket{\psi_{\Thr,i}} + \ket{\psi_{\Thr,i}^\err}.\]

Now consider the following algorithm.

\begin{centering}
\begin{tcolorbox}[
    standard jigsaw,
    opacityback=0,
    width=120mm
]
$\Amp^{O[\bA],O[\bA^\bot]}$:
\begin{itemize}
    \item Take $\ket{\psi_\bA}$ as input.
    \item Compute $\ket{\widetilde{\psi}_{\bA^0}} \coloneqq \Amplify_{\eta,\zeta}^{U_{\ket{\psi_\bA}\bra{\psi_\bA}},U_{\Pi[\bA]_0}}(\ket{\psi_\bA})$.
    \item Sample $i \gets [2^\ell]$.
    \item Compute and output $\ket{\widetilde{\psi}_{\Thr,i}} \coloneqq \Amplify_{\eta,\zeta}^{U_{\ket{\widetilde{\psi}_{\bA^0}}\bra{\widetilde{\psi}_{\bA^0}}},U_{\widetilde{\Thr}[\bA]_i}}(\ket{\widetilde{\psi}_{\bA^0}})$.
\end{itemize}
\end{tcolorbox}
\end{centering}

We first verify that $\Amp$ can be implemented with just access to the collection of oracles $O[\bA]$ and $O[\bA^\bot]$, and we bound the total number of queries that it makes.

\begin{itemize}
    \item Each $U_{\Pi[\bA]_0}$ query requires $t$ queries to the collection of oracles $O[\bA]$.
    \item Each $U_{\ket{\psi_\bA}\bra{\psi_\bA}}$ query requires running $U_\Com^{O[\bA],O[\bA^\bot]}$ in reverse, projecting onto $\ket{\bA}$, and then running $U_\Com^{O[\bA],O[\bA^\bot]}$ forward. This takes a total of $t + \poly(\secp)$ queries to $O[\bA], O[\bA^\bot]$.
    \item Thus, computing $\ket{\widetilde{\psi}_{\bA^0}}$ requires $O((t + \poly(\secp))\log(1/\zeta)/\eta) \leq 2^{2t}$ queries. 
    \item Each $U_{\widetilde{\Thr}[\bA]_i}$ query requires $O(2^{2\ell}(\log{1/\gamma}))$ queries to $\Pi[\bA]_0$ or $\Pi[\bA]_1$, which means at most $2^{49t}$ queries to the collection $O[\bA]$.
    \item Each $U_{\ket{\widetilde{\psi}_{\bA^0}}\bra{\widetilde{\psi}_{\bA^0}}}$ query requires at most $2^{2t+1}$ queries to $O[\bA],O[\bA^\bot]$, by the derivation above.
    \item Thus, computing $\ket{\widetilde{\psi}_{\Thr,i}}$ requires $O(2^{49t}\log(1/\zeta)/\eta) \leq 2^{51t}$ queries to $O[\bA],O[\bA^\bot]$.
\end{itemize}

Next, we verify that each $\Amplify$ procedure is initialized with a state that has sufficient overlap with its target subspace. That is, we need to show that

\begin{enumerate}
    \item $\big\| \Pi[\bA]_0\ket{\psi_\bA}\big\|^2 \geq \eta^2 = \frac{1}{2^{2t}}$, and 
    \item $\big\| \widetilde{\Thr}[\bA]_i\ket{\widetilde{\psi}_{\bA^0}}\big\|^2 \geq \eta^2 = \frac{1}{2^{2t}}.$
\end{enumerate}



Since $(U_\Com,U_\Open)$ violates \cref{claim:worst-case} and $t = 5p$, we have that 

\[\big\| \Pi[\bA]_0\ket{\psi_\bA}\big\|^2 \geq \big\| \Pi[\bA]_1\Pi[\bA]_0\ket{\psi_\bA}\big\|^2 \geq \frac{1}{2^{2p+3}} \geq \frac{1}{2^{2t}}. \]

By the guarantee of \cref{thm:quantum-search}, this implies that $\|\ket{\psi_{\bA^0}^\err}\| \leq \zeta$. Then, we have that 

\begin{align*}
    \big\| \widetilde{\Thr}[\bA]_i\ket{\widetilde{\psi}_{\bA^0}}\big\|^2 &\geq \big\| \widetilde{\Thr}[\bA]_i\ket{\psi_{\bA^0}}\big\|^2 - 2\big \| \ket{\psi_{\bA^0}^\err}\big\| \\
    &\geq \big\| \widetilde{\Thr}[\bA]_i\Thr[\bA]_{\epsilon+1/2^\ell}\ket{\psi_{\bA^0}}\big\|^2 - 2\zeta \\
    &\geq (1-\gamma)\big\| \Thr[\bA]_{\epsilon+1/2^\ell}\ket{\psi_{\bA^0}}\big\|^2 - 2\zeta \\
    &\geq (1-\gamma)\big\| \Thr[\bA]_{\epsilon + 1/2^\ell}\Pi[\bA]_0\ket{\psi_\bA}\big\|^2 - 2\zeta \\
    &= (1-\gamma)\big\| \Thr[\bA]_{\epsilon + 1/2^\ell}\ket{\psi_\bA}\big\|^2 - 2\zeta \\
    &\geq (1-\gamma)\left(\frac{1}{2^{2p+3}} - \epsilon - \frac{1}{2^\ell}\right) - 2\zeta \\
    &\geq (1-\gamma)\left(\frac{1}{2^t}\right) - 2\zeta \\
    &\geq \frac{1}{2^{2t}},
\end{align*}

where the third inequality uses the guarantee of \cref{thm:alternating-projectors}, and the fifth inequality follows from \cref{fact:thr} and the fact that \[\big\|\Pi[\bA]_1\Pi[\bA]_0\ket{\psi_\bA}\big\|^2 \geq \frac{1}{2^{2p+3}}.\]


Finally, our goal will be the show that 

\[\E_{i \gets [2^\ell]}\left[\big\| \Thr[\bA]_\epsilon \ket{\widetilde{\psi}_{\Thr,i}}\big\|^2\right] \geq 1-\frac{1}{2^{10t}}.\]

Towards this, note that for any fixed $i \in [2^\ell]$, 

\begin{align*}
    \big\| \Thr[\bA]_\epsilon \ket{\widetilde{\psi}_{\Thr,i}}\big\|^2
    &= \big\| \Thr[\bA]_\epsilon \left(\ket{\psi_{\Thr,i}} + \ket{\psi_{\Thr,i}^\err}\right)\big\|^2 \\
    &\geq \big\| \Thr[\bA]_\epsilon \ket{\psi_{\Thr,i}}\big\|^2 - 2\big \| \ket{\psi_{\Thr,i}^\err}\big\| \\
    &\geq \frac{\big\|\Thr[\bA]_\epsilon\widetilde{\Thr}[\bA]_i\ket{\widetilde{\psi}_{\bA^0}}\big\|^2}{\big\| \widetilde{\Thr}[\bA]_i\ket{\widetilde{\psi}_{\bA^0}}\big\|^2}- 2\zeta \\
    &= \frac{\big\|\Thr[\bA]_\epsilon\widetilde{\Thr}[\bA]_i(\ket{\psi_{\bA^0}} + \ket{\psi_{\bA^0}^\err})\big\|^2}{\big\| \widetilde{\Thr}[\bA]_i\ket{\widetilde{\psi}_{\bA^0}}\big\|^2}- 2\zeta \\
    &\geq \frac{\big\| \Thr[\bA]_\epsilon \widetilde{\Thr}[\bA]_i \Pi[\bA^0]
    \ket{\psi_\bA}\big\|^2 - 2\big\| \ket{\psi_{\bA^0}^\err}\big\|}{\big\|\widetilde{\Thr}[\bA]_i\ket{\widetilde{\psi}_{\bA^0}} \big\|^2 \big\| \Pi[\bA^0]\ket{\psi_\bA}\big\|^2} - 2\zeta \\
    &\geq \frac{\big\| \Thr[\bA]_\epsilon \widetilde{\Thr}[\bA]_i \Pi[\bA^0]
    \ket{\psi_\bA}\big\|^2 - 2\zeta}{\big\|\widetilde{\Thr}[\bA]_i\ket{\psi_{\bA^0}} \big\|^2 \big\| \Pi[\bA^0]\ket{\psi_\bA}\big\|^2 + 3\big\| \ket{\psi_{\bA^0}^\err}\big\|}- 2\zeta \\
    &\geq \frac{\big\| \Thr[\bA]_\epsilon \widetilde{\Thr}[\bA]_i \Pi[\bA^0]
    \ket{\psi_\bA}\big\|^2 - 2\zeta}{\big\|\widetilde{\Thr}[\bA]_i\Pi[\bA^0]\ket{\psi_\bA}\big\|^2 + 3\zeta}- 2\zeta,
\end{align*}

where the 2nd, 4th, and 5th inequalities use the guarantee of \cref{thm:quantum-search}.

%\takashi{In the 3rd inequality, shouldn't the error term be divided by $\big\| \widetilde{\Thr}[\bA]_i\ket{\widetilde{\psi}_{\bA^0}}\big\|^2$?}
%\takashi{The final line also uses \cref{thm:quantum-search} and should be an inequality.}

Next, since $\Pi[\bA^0]\ket{\psi_\bA} \in \mathsf{Im}(\Pi[\bA^0])$, for any $i \in [2^\ell]$ we can write \[\Pi[\bA^0]\ket{\psi_\bA} \coloneqq \ket{\psi_{i,\high}} + \ket{\psi_{i,\med}} + \ket{\psi_{i,\low}},\] where




%By the fact that $(U_\Com, U_\Open)$ violates \cref{claim:worst-case}, and by the definition of $\mathsf{Jor}[\bA]$, we know that \[\bigg\| \mathsf{Jor}[\bA]_\beta \ket{\psi_\bA}\bigg\|^2 \geq \frac{1}{2^{2p+3}} - \beta \geq \frac{1}{2^{3p}}.\] Thus, by \cref{thm:alternating-projectors}, we have that for any $i \in [2^{t'}]$, \[\bigg\|\Pi[\mathsf{Th}]_i \ket{\psi_\bA} \bigg\|^2 \geq \frac{1}{2^{3p}} - \gamma \coloneqq \eta.\] For $i \in [2^{t'}]$, define \[\ket{\psi_{i,\bA}} \coloneqq \mathsf{Amplify}^{U_{\ket{\psi_\bA}\bra{\psi_\bA}},U_{\Pi[\mathsf{Th}]_i}}(\ket{\psi_{\bA}}),\] and define \[\ket{\psi_{i,\mathsf{target}}} \coloneqq \frac{\Pi[\mathsf{Th}]_i\ket{\psi_\bA}}{\|\Pi[\mathsf{Th}]_i\ket{\psi_\bA}\|}.\] Then by \cref{thm:quantum-search}, we have that \[\braket{\psi_{i,\mathsf{target}}|\psi_{i,\bA}}^2 \geq 1-1/2^{T\eta^2}.\]


\begin{itemize}
    \item $\ket{\psi_{i,\high}}$ is supported on right singular vectors of $\Pi[\bA]_1\Pi[\bA]_0$ with singular value $s$ such that \[s^2 \geq \epsilon + i/2^{2\ell},\]
    \item $\ket{\psi_{i,\med}}$ is supported on right singular vectors of $\Pi[\bA]_1\Pi[\bA]_0$ with singular value $s$ such that \[\epsilon + i/2^{2\ell} > s^2 > \epsilon + (i-1)/2^{2\ell},\]
    \item and $\ket{\psi_{i,\low}}$ is supported on right singular vectors of $\Pi[\bA]_1\Pi[\bA]_0$ with singular value $s$ such that \[\epsilon + (i-1)/2^{2\ell} \geq s^2.\]
\end{itemize}

By \cref{thm:alternating-projectors}, we have that \[\|\widetilde{\Thr}[\bA]_i\ket{\psi_{i,\low}}\|^2 \leq \gamma.\] 

Also, defining $\ket{\widehat{\psi}_{i,\high}} \coloneqq \ket{\psi_{i,\high}} / \big\| \ket{\psi_{i,\high}}\big\|$ to be the normalized state $\ket{\psi_{i,\high}}$, and noting that by Gentle Measurement (\cref{lemma:gentle-measurement}) and \cref{thm:alternating-projectors}, 

\[\TD\left(\frac{\widetilde{\Thr}[\bA]_i\ket{\widehat{\psi}_{i,\high}}}{\big\| \widetilde{\Thr}[\bA]_i\ket{\widehat{\psi}_{i,\high}}\big\| }, \ket{\widehat{\psi}_{i,\high}}\right) \leq 2\sqrt{\gamma},\]

we can bound

\begin{align*}
    \big\| \Thr[\bA]_\epsilon\widetilde{\Thr}[\bA]_i\ket{\psi_{i,\high}}\big\|^2 &= \big\| \Thr[\bA]_\epsilon\widetilde{\Thr}[\bA]_i\ket{\widehat{\psi}_{i,\high}}\big\|^2 \big\| \ket{\psi_{i,\high}}\big\|^2 \\ 
    &= \bigg\| \Thr[\bA]_\epsilon \frac{\widetilde{\Thr}[\bA]_i\ket{\widehat{\psi}_{i,\high}}}{\big\| \widetilde{\Thr}[\bA]_i\ket{\widehat{\psi}_{i,\high}}\big\| }\bigg\|^2 \big\| \widetilde{\Thr}[\bA]_i\ket{\widehat{\psi}_{i,\high}}\big\|^2 \big\| \ket{\psi_{i,\high}}\big\|^2 \\
    &\geq \left(\big\| \Thr[\bA]_\epsilon \ket{\widehat{\psi}_{i,\high}}\big\|^2 - 2\sqrt{\gamma}\right)\big\| \widetilde{\Thr}[\bA]_i\ket{\widehat{\psi}_{i,\high}}\big\|^2 \big\| \ket{\psi_{i,\high}}\big\|^2 \\
    &\geq (1-2\sqrt{\gamma})(1-\gamma)\big\|\ket{\psi_{i,\high}}\|^2 \\
    &\geq (1-3\sqrt{\gamma})\big\| \ket{\psi_{i,\high}}\big\|^2,
\end{align*}

where the second inequality uses the guarantee of \cref{thm:alternating-projectors}.

Thus, for any $i \in [2^\ell]$, we have that  

\begin{align*}
\big\| \Thr[\bA]_\epsilon \ket{\widetilde{\psi}_{\Thr,i}}\big\|^2 
&\geq \frac{\big\| \Thr[\bA]_\epsilon \widetilde{\Thr}[\bA]_i (\ket{\psi_{i,\high}} + \ket{\psi_{i,\med}} + \ket{\psi_{i,\low}})\big\|^2 - 2\zeta}{\big\|\widetilde{\Thr}[\bA]_i(\ket{\psi_{i,\high}} + \ket{\psi_{i,\med}} + \ket{\psi_{i,\low}})\big\|^2 + 3\zeta}- 2\zeta \\
&\geq \frac{\big\|\Thr[\bA]_\epsilon\widetilde{\Thr}[\bA]_i\ket{\psi_{i,\high}}\big\|^2 - 4\big\|\ket{\psi_{i,\med}}\big\| - 2\big\|\ket{\psi_{i,\low}}\big\| - 2\zeta}{\big\|\ket{\psi_{i,\high}}\big\|^2 + 5\big\|\ket{\psi_{i,\med}}\big\| + 3\big\|\ket{\psi_{i,\low}}\big\| + 3\zeta} - 2\zeta \\
&\geq \frac{(1-3\sqrt{\gamma})\big\|\ket{\psi_{i,\high}}\big\|^2 - 4\big\| \ket{\psi_{i,\med}}\big\| - 2\sqrt{\gamma} - 2\zeta}{\big\| \ket{\psi_{i,\high}}\big\|^2 + 5\big\| \ket{\psi_{i,\med}}\big\| + 3\sqrt{\gamma} + 3\zeta} - 2\zeta \\
&\geq (1-3\sqrt{\gamma})\left(1 - \frac{5\big\| \ket{\psi_{i,\med}}\big\| + 3\sqrt{\gamma} + 3\zeta}{\big\| \ket{\psi_{i,\high}}\big\|^2}\right) - \frac{4 \big\| \ket{\psi_{i,\med}}\big\| +2\sqrt{\gamma} + 2\zeta}{\big\| \ket{\psi_{i,\high}}\big\|^2} - 2\zeta \\ 
&\geq 1-\frac{9\big\| \ket{\psi_{i,\med}}\big\| + 5\sqrt{\gamma} + 5\zeta}{\big\|\ket{\psi_{i,\high}}\big\|^2} - 2\zeta.
\end{align*}

Noting that \[\big\| \ket{\psi_{i,\high}}\big\|^2 \geq \big\| \Thr[\bA]_{\epsilon + 1/2^\ell}\Pi[\bA]_0\ket{\psi_\bA}\big\|^2 \geq \frac{1}{2^{2p+3}} - \epsilon - \frac{1}{2^\ell} \geq \frac{1}{2^{3p}},\] and, since the $\{\ket{\psi_{i,\med}}\}_{i \in [2^\ell]}$ are pairwise orthogonal, \[\E_{i \gets [2^\ell]}\left[\big\| \ket{\psi_{i,\med}}\big\|^2\right] \leq \frac{1}{2^\ell},\] we can conclude that 

\begin{align*}
\E_{i \gets [2^\ell]}&\left[\big\| \Thr[\bA]_\epsilon \ket{\widetilde{\psi}_{\Thr,i}}\big\|^2\right]\\ 
&\geq 1-2^{3p}\left(\frac{9}{2^{\ell/2}} + 5\sqrt{\gamma} + 5\zeta\right) - 2\zeta \\
&\geq 1 - \frac{9 \cdot 2^t}{2^{12t}} - \frac{5 \cdot 2^t}{2^{12t}} - \frac{5 \cdot 2^t}{2^{12t}} - \frac{2}{2^{12t}}\\
&\geq 1 - \frac{1}{2^{10t}}.
\end{align*}

To wrap up the proof of the claim, we first see that by Markov,

\[\Pr_{i \gets [2^\ell]}\left[\big\| \Thr[\bA]_\epsilon \ket{\widetilde{\psi}_{\Thr,i}}\big\|^2  \geq 1-\frac{1}{2^{5t}}\right] \geq 1 - \frac{1}{2^{5t}}.\]

Now, let $\mathsf{U}\text{-}\Amp^{O[\bA],O[\bA^\bot]}$ be the purification of $\Amp^{O[\bA],O[\bA^\bot]}$, and define 

\[\widetilde{U}_\Com^{O[\bA],O[\bA^\bot]} \coloneqq \mathsf{U}\text{-}\Amp^{O[\bA],O[\bA^\bot]}U_\Com^{O[\bA],O[\bA^\bot]}.\] Then it follows that

\[\bigg\| \Thr[\bA]_\epsilon \widetilde{U}_\Com^{O[\bA],O[\bA^\bot]}(\ket{\bA})\bigg\|^2 \geq \left(1-\frac{1}{2^{5t}}\right)^2 \geq 1-\frac{1}{2^{4t}}.\] Recalling from above that $\Amp$ makes at most $2^{51t}$ oracle queries completes the proof.


 
%We write \[\Pi[\mathsf{Th}]_i\ket{\psi_{i,\high}} \coloneqq \ket{\psi_{i,\mathsf{Jor}}} + \ket{\psi^\bot_{i,\mathsf{Jor}}},\] where \[\ket{\psi_{i,\mathsf{Jor}}} = \mathsf{Jor}[\bA]_\epsilon\Pi[\mathsf{Th}]_i\ket{\psi_{i,\high}},\] and define \[\ket{\psi_{i,\bad}} \coloneqq \ket{\psi^\bot_{i,\mathsf{Jor}}} + \Pi[\mathsf{Th}]_i\ket{\psi_{i,\med}} + \Pi[\mathsf{Th}]_i\ket{\psi_{i,\low}}.\]
   % Then for any $i \in [2^{\ell}]$, we have that 
    %\begin{align*}
        %\big\| \mathsf{Jor}[\bA]_\epsilon \ket{\psi_{i,\mathsf{target}}}\big\|^2 &= \frac{\big\| \mathsf{Jor}[\bA]_\epsilon\Pi[\mathsf{Th}]_i(\ket{\psi_{i,\high}} + \ket{\psi_{i,\med}} + \ket{\psi_{i,\low}})\big\|^2}{\big\| \Pi[\mathsf{Th}]_i(\ket{\psi_{i,\high}} + \ket{\psi_{i,\med}} + \ket{\psi_{i,\low}})\big\|^2} \\
        %&\geq \frac{\big\| \ket{\psi_{i,\mathsf{Jor}}}\big\|^2}{\big\| \ket{\psi_{i,\mathsf{Jor}}} + \ket{\psi_{i,\mathsf{bad}}}\big\|^2} \\
        %&\geq 1 - \frac{3\big\| \ket{\psi_{i,\mathsf{bad}}}\big\|^2}{\big\| \ket{\psi_{i,\mathsf{Jor}}}\big\|^2}.
    %\end{align*}
    
    
%Next, we see that for any $i \in [2^{\ell}]$, 
%\begin{align*}
%\big\| \ket{\psi_{i,\mathsf{Jor}}}\big\|^2 &= \big\| \mathsf{Jor}[\bA]_\epsilon\Pi[\mathsf{Th}]_i\ket{\psi_{i,\high}} \big\|^2 = \big\| \Pi[\mathsf{Th}]_i\mathsf{Jor}[\bA]_\epsilon\ket{\psi_{i,\high}} \big\|^2 \\
%&= \big\| \Pi[\mathsf{Th}]_i\ket{\psi_{i,\high}}\big\|^2 \geq (1-\gamma) \big\| \ket{\psi_{i,\high}}\big\|^2 \geq (1-\gamma)(1/2^{2p+3}-\epsilon),
%\end{align*} and \[\E_{i \gets [2^{\ell}]}\left[\big\|\ket{\psi_{i,\mathsf{bad}}} \big\|^2\right] \leq \frac{5}{2^\ell} + 4\gamma.\]

%Then, we have that 
    %\begin{align*}
        %\E_{i \gets [2^{\ell}]}&\left[\bigg\| \mathsf{Jor}[\bA]_\epsilon \mathsf{Amplify}^{U_{\ket{\psi_\bA}\bra{\psi_\bA}},U_{\Pi[\mathsf{Th}]_i}}(\ket{\bA})\bigg\|^2\right] \\ 
        %&\geq \E_{i \gets [2^{\ell}]}\left[\bigg\|\mathsf{Jor}[\bA]_\epsilon\ket{\psi_{i,\mathsf{target}}}\bra{\psi_{i,\mathsf{target}}}\ket{\psi_{i,\bA}}\bigg\|^2\right] \\ 
        %&\geq \left(1-\frac{1}{2^{T\eta^2}}\right)\E_{i \gets [2^{\ell}]}\left[\bigg\| \mathsf{Jor}[\bA]_\epsilon \ket{\psi_{i,\mathsf{target}}}\bigg\|^2\right] \\
        %&\geq \left(1-\frac{1}{2^{T\eta^2}}\right)\left(1-\frac{5/2^\ell + 4\gamma}{(1-\gamma)(1/2^{2p+3}-\epsilon)}\right) \coloneqq 1-\nu.
    %\end{align*}


%Next, we note that $\mathsf{Amplify}$'s oracle queries can be answered with access to only the collection of oracles $O[\bA]$ and $O[\bA^\bot]$, and we analyze the number of queries to $O[\bA]$ and $O[\bA^\bot]$ that $\mathsf{Amplify}$ makes. 
    %\begin{itemize}
        %\item Each query to $U_{\ket{\psi_\bA}\bra{\psi_\bA}}$ requires running $U_\Com^{O[\bA],O[\bA^\bot]}$ in reverse, projecting onto $\ket{\bA}$, and then running $U_\Com^{O[\bA],O[\bA^\bot]}$ forward. Since each of these steps takes $U_\Com$ makes $\poly(\secp)$ queries, and projecting onto $\ket{\bA}$ takes $t$ queries, this takes $t + \poly(\secp)$ queries in total.
        %\item Each query to $U_{\Pi[\mathsf{Th}]_i}$ takes $O\left(\frac{\log(1/\gamma)\sqrt{\beta}}{(1/2^{2\ell})}\right)$ queries to $\Pi[\bA]_0$ or $\Pi[\bA]_1$, so the total number of queries to the oracles $O[\bA]$ is bounded by $O(T \cdot t \cdot \log(1/\gamma) \cdot 2^{2\ell})$. This is the dominant term, so we use it to bound the total number of queries made by $\mathsf{Amplify}$.
    %\end{itemize}
    
    
%By Markov, we have that 
    %\begin{align*}
        %\Pr_{i \gets [2^{\ell}]}\left[\bigg\| \mathsf{Jor}[\bA]_\epsilon \mathsf{Amplify}^{U_{\ket{\psi_\bA}\bra{\psi_\bA}},U_{\Pi[\mathsf{Th}]_i}}(\ket{\bA})\bigg\|^2 \geq 1-\sqrt{\nu}\right] \geq 1-\sqrt{\nu}.
    %\end{align*}
    %Finally, we define the algorithm $\mathsf{Samp}\text{-}\mathsf{Amplify}^{O[\bA],O[\bA^\bot]}$ to be a purification of the procedure that samples $i \gets [2^{\ell}]$ and runs $\mathsf{Amplify}^{U_{\ket{\psi_\bA}\bra{\psi_\bA}},U_{\Pi[\mathsf{Th}]_i}}(\ket{\bA})$. Then it holds that \[\bigg\| \mathsf{Jor}[\bA]_\epsilon \mathsf{Samp}\text{-}\mathsf{Amplify}^{O[\bA],O[\bA^\bot]}(\ket{\bA})\bigg\|^2 \geq 1-2\sqrt{\nu}.\]






%Define some $\epsilon,\delta,\gamma$ based on $p(\secp),t(\secp)$, and $n(\secp)$, and define $P^{\Pi_\bS^0,U_\cA^\dagger \Pi_\bS^1 U_\cA}_{\epsilon,\delta,\gamma}$ to be \[{U[\mathsf{Threshold}]^{\Pi_\bS^0,U_\cA^\dagger \Pi_\bS^1 U_\cA}_{\epsilon,\delta,\gamma}}^\dagger \ket{1}\bra{1} U[\mathsf{Threshold}]^{\Pi_\bS^0,U_\cA^\dagger \Pi_\bS^1 U_\cA}_{\epsilon,\delta,\gamma},\] where $U[\mathsf{Threshold}]^{\Pi_\bS^0,U_\cA^\dagger \Pi_\bS^1 U_\cA}_{\epsilon,\delta,\gamma}$ is a unitary implementation of the algorithm $\mathsf{Threshold}^{\Pi_\bS^0,U_\cA^\dagger \Pi_\bS^1 U_\cA}_{\epsilon,\delta,\gamma}$.

%Then, by amplitude amplification, it suffices to prove the following, for some appropriately defined $f(\secp)$ and $\nu(\secp)$.

%Now, set $A = M[\bS]_A$ and $B = M[\bS]_B$, and given parameters $(\epsilon,\delta,\gamma)$ and $i \in [2^t]$, define $P_i$ to be a projection onto vectors accepted by the algorithm $\mathsf{Threshold}_{\epsilon-i/2^{2t},1/2^{2t},\gamma}^{U_A,U_B}$. Then, by sampling $i \gets [2^t]$, and running $\mathsf{Amplify}^{U_{\ket{\psi_\bS}\ket{0}},U_{P_i}}$ with enough iterations, we can produce a state $\ket{\psi'_\bS}$ that is $(1-1/2^{2t})$-close to $\mathsf{Jor}[\bS]_{\epsilon-2^{t}}$. 

%\takashi{This sentence was not clear to me. Do you mean that the procedure works for an overwhelming fraction of $i$?} \james{I think we can work with expectations, but I will update this proof next and hopefully clear up the question} 


\end{proof}



%\begin{lemma}
%There does not exist any two-part quantum algorithm $(\cA,U_\cA)$, where $\cA$ issues $f(\secp)$ queries to two oracles and outputs a state on a $k$-qubit register where $k\geq n$, and $U_\cA$ is a $k$-qubit unitary, such that for all $\bS \in \SSC.\Gen^{2/3}(1^\secp,t,n)$ it holds that \[\bra{\psi_\bS}P^{\Pi_\bS^0,U_\cA^\dagger \Pi_\bS^1 U_\cA}_{\epsilon,\delta,\gamma}\ket{\psi_\bS} \geq 1-\nu(\secp),\] where $\ket{\psi_{\bS}} \coloneqq \cA^{O_\bS,O_\bS^\bot}(\ket{\bS})$.
%\end{lemma}

Finally, we prove \cref{claim:jor}, which, as we have shown, suffices to prove \cref{thm:binding}.

\begin{proof}(of \cref{claim:jor}) We will use the following imported theorem.

\begin{importedtheorem}[\cite{10.1145/2213977.2213983}]\label{thm:adversary-method}
Let $\cO$ be a set of classical functionalities $F : \{0,1\}^* \to \{0,1\}$. Let $\cR$ be a symmetric binary relation between functionalities where for every $F \in \cO$, $(F,F) \notin \cR$, and for every $F \in \cO$, there exists $G \in \cO$ such that $(F,G) \in \cR$. Moreover, for any $F \in \cO$ and $x$ such that $F(x) = 0$, suppose that \[\Pr_{G \gets \cR_F}[G(x) = 1] \leq \epsilon,\] where $\cR_F$ is the set of $G$ such that $(F,G) \in \cR$. Now, consider any oracle-aided unitary $U^F(\ket{\psi_F})$ that has oracle access to some $F \in \cO$, is initialized with some state $\ket{\psi_F}$ that may depend on $F$, makes $T$ queries, and outputs a state $\ket{\widetilde{\psi}_F}$. Then if $|\braket{\psi_F | \psi_G}| \geq c$ for all $(F,G) \in \cR$ and $\E_{(F,G) \gets \cR}[|\braket{\widetilde{\psi}_F|\widetilde{\psi}_G}|] \leq d$, then $T = \Omega\left(\frac{c-d}{\sqrt{\epsilon}}\right)$.
\end{importedtheorem}


Now, suppose there exists $(U_\Com, U_\Open)$ that violates \cref{claim:jor}. Recall that $U_\Com$ has access to the collection of $2t$ oracles $O[\bA]$ and $O[\bA^\bot]$, defined by the sequence of affine subspaces $(A_1,\dots,A_t) = (S_1+v_1,\dots,S_t+v_t)$, where each is a $n/2$ dimensional affine subspace of $\bbF_2^{3n/4}$. We define a single oracle $F_\bA$ that takes as input $(i,b,s)$ and if $b=0$ outputs whether $s \in S_i + v_i$, and if $b=1$ outputs whether $s \in S_i^\bot$.

Then, we define a binary symmetric relation on oracles $F_\bA, F_\bB$ as follows. Letting $\bA = (A_1,\dots,A_t) = (S_1+v_1,\dots,S_t + v_t)$ and $\bB = (B_1,\dots,B_t) = (T_1+w_1,\dots,T_t+w_t)$ we define $(F_\bA,F_\bB) \in \cR$ if and only if for all $i \in [t]$ and $b \in \{0,1\}$, it holds that $\mathsf{dim}(A_i^b \cap B_i^b) = n/2 - 2$. That is, for each pair of $n/2$ dimensional affine subspaces $A_i$ and $B_i$, the intersection of $A_i^0$ and $B_i^0$ has $n/2-2$ dimensions, and the intersection of $A_i^1$ and $B_i^1$ also has $n/2-2$ dimensions. Note that this means that the intersection of $A_i$ and $B_i$ has $n/2-1$ dimensions.

Given $\cR$ defined this way, we see that for any fixed $F_\bA$ and $(i,b,s)$ such that $F_\bA(i,b,s) = 0$,

\begin{align*}
    \Pr_{F_\bB \gets \cR_{F_\bA}}&[F_\bB(i,b,s) = 1] \\ &\leq \max_i\left\{\max\left\{\frac{|B_i \setminus A_i|}{|\bbF_2^{3n/4} \setminus A_i \setminus \{0^{3n/4}\}|},\frac{|T_i^\bot \setminus S_i^\bot|}{|\bbF_2^{3n/4} \setminus S_i^\bot|}\right\}\right\} \\ &\leq \max\left\{\frac{2^{n/2-1}}{2^{3n/4} - 2^{n/2} - 1}, \frac{2^{n/4-1}}{2^{3n/4}-2^{n/4}}\right\}\\ &\leq \frac{1}{2^{n/4}}.
\end{align*}

Next, we note that $U_\Com^{F_\bA}$ is initialized with the state $\ket{\bA}$, and, for any $(\bA,\bB)$ such that $(F_\bA,F_\bB) \in \cR$, it holds that $|\braket{\bA|\bB}| = (1/2)^t$. Our goal is then the bound \[\E_{(F_\bA,F_\bB) \gets \cR}\left[|\braket{\psi_\bA | \psi_\bB}|\right],\] where $\ket{\psi_\bA} \coloneqq U_\Com^{F_\bA}(\ket{\bA})$. For each $\ket{\psi_\bA}$, we write $\ket{\psi_\bA} \coloneqq \ket{\psi_\bA^\Thr} + \ket{\psi_\bA^\err}$, where $\ket{\psi_\bA^\Thr} \coloneqq \Thr[\bA]_{1/2^{3p}}\ket{\psi_\bA}$. By the fact that $(U_\Com, U_\Open)$ violates \cref{claim:jor}, we know that $\big\| \ket{\psi_\bA^\err} \big\|^2 \leq 1/2^{4t}$. Thus, we have that \[\E_{(F_\bA,F_\bB) \gets \cR}[|\braket{\psi_\bA | \psi_\bB}] \leq \E_{(F_\bA,F_\bB) \gets \cR}[|\braket{\psi_\bA^\Thr | \psi_\bB^\Thr}|] + 3/2^{2t}.\]

Continuing, we can bound 


\begin{tcolorbox}[
    standard jigsaw,
    opacityback=0
]
We want to show that \[\E_{F_\bA,F_\bB}[|\braket{\psi_\bA^\Thr | \psi_\bA^\Thr}|] \leq \frac{1}{\epsilon} \cdot \frac{1}{2^{2t}},\] so that we obtain an approximately $1/2^t$ decrease in expected inner product from $|\braket{\psi_\bA | \psi_\bB}| = 1/2^t$. I was hoping to intuitively follow \cite{arxiv:BenSat16}, page 27, who show the following. For $S < \bbF_2^n$, they consider the subspace (I'll call it $\mathsf{Im}(\Pi_S)$) supported on $(s,s')$ such that $s \in S$ and $s' \in S^\bot$. Then they show that for any set of vectors  $\{\ket{\psi_S}\}_{S}$ where each $\ket{\psi_S} \in \mathsf{Im}(\Pi_S)$, that $\E_{S,T}[\braket{\psi_S | \psi_T}] \leq 1/4$, where the expectation is over $S,T$ that share $n/2-1$ dimensions. In their proof, they are essentially able to bound \[\E_{S,T}[\braket{\psi_S | \psi_T}] \leq \E_{S,T}[\|\Pi_T \ket{\psi_S}\|^2],\] and then show that given any $(s,s') \in (S,S^\bot)$, the probability that $s \in T$ and $s' \in T^\bot$ is 1/4.

I was hoping to do something similar here, and start by bounding 

\[\E_{(F_\bA,F_\bB)}[|\braket{\psi_\bA^\Thr | \psi_\bB^\Thr}|] \leq \max_{\bA, \ket{\psi_\bA^\Thr}}\E_{F_\bB \gets \cR_{F_\bA}}\left[\big\| \Thr[\bB]_\epsilon\ket{\psi_\bA^\Thr}\big\|^2\right].\] If that is true, then the rest of the proof works, because we get a $1/\epsilon$ term from going from $\Thr$ to $\Pi[\bB]_1\Pi[\bB]_0$, and a $1/2^t$ term from each of these projectors. 

However, unlike the \cite{arxiv:BenSat16} setting, I don't think that claim is true, and we can only say that 

\[\E_{(F_\bA,F_\bB)}[|\braket{\psi_\bA^\Thr | \psi_\bB^\Thr}|] \leq \max_{\bA, \ket{\psi_\bA^\Thr}}\E_{F_\bB \gets \cR_{F_\bA}}\left[\big\| \Thr[\bB]_\epsilon\ket{\psi_\bA^\Thr}\big\|\right].\] This is not good enough, because it would give a final bound $> 1/2^t$, which is useless. 

Or we can say that \[\E_{(\bA,\bB)}[|\braket{\psi_\bA^\Thr | \psi_\bB^\Thr}|] \leq \frac{1}{\epsilon^2}\E_{(\bA,\bB)}[|\bra{\psi_\bA^\Thr}\Pi[\bA]_1\Pi[\bA]_0\Pi[\bB]_0\Pi[\bB]_1\ket{\psi_\bB^\Thr}|],\] but then the $\Pi[\bA]_0$ and $\Pi[\bA]_1$ don't commute (recall $\Pi[\bA]_1 = U^\dagger\Pi[\bA^1]U$ for some arbitrary $U$). I think the difference here is that in \cite{arxiv:BenSat16}, all their subspaces $\Pi_S$ are just diagonal in the standard basis and they immediately consider the intersections of the subspaces (their sums over $(a,b) \in \Lambda(A) \cup \Lambda(B)$), and then apply a Cauchy-Shwartz step. In our case, the subspaces $\Thr[\bA]_\epsilon$ don't all commute with each other.

We at least know that since $\Thr[\bA]_\epsilon$ is contained in $\Pi[\bA]_0$, we could bound \[\E_{F_\bA,F_\bB}[|\braket{\psi_\bA^\Thr | \psi_\bA^\Thr}|] \leq \frac{1}{2^{t}},\] by using the fact that each $\ket{\psi_\bA^\Thr} \in \mathsf{Im}(\Pi[\bA]_0)$, and exactly following the proof in \cite{arxiv:BenSat16}. But we also somehow want to use the stronger condition that each $\ket{\psi_\bA^\Thr} \in \mathsf{Im}(\Thr[\bA]_\epsilon)$, which I was hoping would give us some way to decrease the expected inner product further by looking at the $\Pi[\bA]_1$ subspaces in addition to $\Pi[\bA]_0$. However, I haven't yet been able to figure out how to do this without taking the square root loss above, making the argument useless. Note that if we show something like 

\[\E_{F_\bA,F_\bB}[|\braket{\psi_\bA^\Thr | \psi_\bA^\Thr}|] \leq \frac{1}{\epsilon} \cdot \frac{1}{2^{3t/2}},\] that would be good enough, but again I don't see yet how to go beyond $1/2^t$. 

\end{tcolorbox}





\[\E_{(F_\bA,F_\bB)}[|\braket{\psi_\bA^\Thr | \psi_\bB^\Thr}|] \leq \max_{\bA, \ket{\psi_\bA^\Thr}}\E_{F_\bB \gets \cR_{F_\bA}}\left[\big\| \Thr[\bB]_{1/2^{3p}}\ket{\psi_\bA^\Thr}\big\|^2\right],\] so from now one, we fix some $\bA$ and a state $\ket{\psi_\bA^\Thr}$ that may depend arbitrarily on $\bA$. Then by \cref{fact:thr}, we have that 

\[\E_{F_\bB \gets \cR_{F_\bA}}\left[\big\| \Thr[\bB]_{1/2^{3p}}\ket{\psi_\bA^\Thr}\big\|^2\right] \leq 2^{3p} \cdot \E_{F_\bB \gets \cR_{F_\bA}}\left[\big\| \Pi[\bB]_1\Pi[\bB]_0\ket{\psi_\bA^\Thr}\big\|^2\right]. \]

Now, we imagine sampling $\bB$ in two steps, as follows. First, we recall that for any affine subspace $A$, both $A^0$ and $A^1$ are affine subspaces. Now, for each $i \in [t]$, we will first sample $B_i^0$ as an affine subspace such that $\mathsf{dim}(A_i^0 \cap B_i^0) = n/2-2$. We denote by $\bB^0$ the resulting sequence of affine subspaces. Since for any $s \in A_i, \Pr[s \in B_i] = 1/2$, and for any $s \notin A_i, \Pr[s \in B_i] < 1/2$, we have that

\[\E_{\bB^0}\left[\big\|\Pi[\bB]_0\ket{\psi_\bA^\Thr}\big\|^2\right] = \E_{\bB^0}\left[\big\|\Pi[\bB^0]\ket{\psi_\bA^\Thr}\big\|^2\right] \leq \left(\max_{i \in [t], s \in \bbF_2^{3n/4}}\Pr\left[s \in B_i^0\right]\right)^t \leq \frac{1}{2^t},\] where the first inequality is due to \cref{claim:max-prob}. Next, for each $i \in [t]$, given fixed $\bA$ and $\bB^0$, we sample $B_i^1$ such that $B_i^0 \union B_i^1$ is an affine subspace, and $\mathsf{dim}(A_i^1 \cap B_i^1) = n/2-2$. For each $i$, we claim that, given $A_i$ and $B_i^0$, there are exactly two disjoint choices for $B_i^1$. To see this, we recall that $A_i^0$ is an affine subspace and $A_i^1 \coloneqq A_i^0 + x$ is a shift of $A_i^0$. Since $B_i^0$ is also an affine subspace, $A_i^0 \cap B_i^0$ is an affine subspace, which we write as a coset $S+u$ of some $n/2-2$ dimensional subspace $S$. Thus, we can write $A_i^0 \coloneqq (S+u) \union (S+u+v)$, $B_i^0 \coloneqq (S+u) \union (S+u+w)$, and $A_i^1 \coloneqq (S+u+x) \union (S+u+v+x)$. Then, $B_i^1$ must be either $(S+u+x) \union (S+u+x+w)$ or $(S+u+v+x) \union (S+u+v+x+w)$, which are disjoint because $v \neq w$.
Thus, we conclude that for any $\ket{\psi}$ that may depend arbitrarily on $\bA$ and $\bB^0$,

\[\E_{\bB^1}\left[\big\|\Pi[\bB]_1\ket{\psi}\big\|^2\right] = \E_{\bB^1}\left[\big\|\Pi[\bB^1]U_\Open \ket{\psi} \big\|^2\right] \leq \left(\max_{i \in [t], s \in \bbF_2^{3n/4}}\Pr\left[s \in B_i^1\right]\right)^t \leq \frac{1}{2^t},\] where the first inequality is due to \cref{claim:max-prob}. Putting it together, we can bound \[\E_{(F_\bA,F_\bB) \gets \cR}\left[|\braket{\psi_\bA | \psi_\bB}|\right] \leq \frac{2^{3p} + 3}{2^{2t}},\]

which, by \cref{thm:adversary-method} implies that $U_\Com$ must be making

\[\Omega\left(2^{n/8} \cdot \left(\frac{1}{2^t} - \frac{2^{3p}+3}{2^{2t}}\right)\right) = \Omega\left(2^{n/8 - 6p}\right) =  \Omega\left(2^{n/8 - 2t}\right) = \Omega\left(2^{60t}\right)\] oracle queries, since $t = 5p$, and $n = 500t$. However, this is a contradiction, as $U_\Com$ was assumed to be making at most $2^{51t}$ oracle queries. This completes the proof.

\subsection{Special case}

\begin{itemize}
    \item Let $U^{\sX,\sY}$ be a unitary on $2^{n+m}$ dimensions, where register $\sX$ is $n$ dimensions and register $\sY$ is $m$ dimensions. 
    \item For any $d$ dimensional affine subspace $A = S+v$ of $\bbF_2^n$, and $b \in \{0,1\}$, let $\Pi_{A^b}^{\sX}$ be the projection onto vectors in $S+v$ that start with $b$. Then let \[\Pi_{A,0}^{\sX,\sY} \coloneqq \Pi_{A^0}^{\sX} \otimes \bbI^\sY, \ \ \, \Pi_{A,1}^{\sX,\sY} \coloneqq U^\dagger(\Pi_{A^1}^{\sX} \otimes \bbI^\sY)U.\]
    \item Suppose that for all $A$, there exists $\ket{\psi_A}^{\sX,\sY} \in \Pi_{A,0} \cap \Pi_{A,1}$, and fix any set of such $\{\ket{\psi_A}\}_A$.
    \item Let $\cR$ be such that $(A,B) \in \cR$ iff $\dim(A^0 \cap B^0) = d-2$ and $\dim(A^1 \cap B^1) = d-2$.
    \item Then, is \[\E_{(A,B) \in \cR}[\braket{\psi_A | \psi_B}] < 1/2?\]
\end{itemize}

I think that to prove this for any $d,n$, it would suffice to prove the case where $d'=2$ and $n' = n-d+2$ (by considering the subspace of cosets of $A^0 \cap B^0$). So fix $d=2$ and arbitrary $n$. To simplify further, lets only randomized over cosets of some fixed 1 dimensional spaces. Consider the following setup.

\begin{itemize}
    \item Fix any $v_A \neq v_B \neq 0^n \in \bbF_2^n$ such that $v_A$ and $v_B$ both start with 0.
    \item Let $\co_0(v_A)$ be the set of $2^{n-2}$ coset representatives of $\{0^n,v_A\}$ that start with 0, let $\co_1(v_A)$ be the set of $2^{n-2}$ coset representatives of $\{0^n,v_A\}$ that start with 1, and define $\co_0(v_B)$ and $\co_1(v_B)$ analogously.
    \item We associate affine subspaces $A$ with $(w_0,w_1) \in  \co_0(v_A) \times \co_1(v_A)$, where $A = \{w_0,w_0+v_A,w_1,w_1+v_A\}$, and affine subspaces $B$ with $(x_0,x_1) \in  \co_0(v_B) \times \co_1(v_B)$, where $B = \{x_0,x_0+v_B,x_1,x_1+v_B\}$.
    \item Then for any $A = (w_0,w_1)$, \[\Pi_{A,0} \coloneqq (\ketbra{w_0}{w_0} + \ketbra{w_0+v_A}{w_0+v_A})^{\sX} \otimes \bbI^\sY, \ \ \, \Pi_{A,1} \coloneqq U^\dagger((\ketbra{w_1}{w_1} + \ketbra{w_1+v_A}{w_1+v_A})^{\sX} \otimes \bbI^\sY)U,\] and for any $B = (x_0,x_1)$, \[\Pi_{B,0} \coloneqq (\ketbra{x_0}{x_0} + \ketbra{x_0+v_B}{x_0+v_B})^{\sX} \otimes \bbI^\sY, \ \ \, \Pi_{B,1} \coloneqq U^\dagger((\ketbra{x_1}{x_1} + \ketbra{x_1+v_B}{x_1+v_B})^{\sX} \otimes \bbI^\sY)U.\]
    \item Let $\cR$ be such that $(A,B) \in \cR$ iff, writing $A = \{w_0,w_0+v_A,w_1,w_1+v_A\}$ and $B = \{x_0,x_0+v_B,x_1,x_1+v_B\}$, we have that $|\{w_0,w_0+v_A\} \cap \{x_0,x_0+v_B\}| = 1$ and $|\{w_1,w_1+v_A\} \cap \{x_1,x_1+v_B\}| = 1$.
    \item Suppose that for all $A$, there exists $\ket{\psi_A}^{\sX,\sY} \in \Pi_{A,0} \cap \Pi_{A,1}$, and for all $B$, there exists $\ket{\psi_B}^{\sX,\sY} \in \Pi_{B,0} \cap \Pi_{B,1}$. Then, is \[\E_{(A,B) \in \cR}[\braket{\psi_A | \psi_B}] < 1/2?\]
    
\end{itemize}

Intuition:

\begin{itemize}
    \item Since $\{\Pi_{A,0}\}$ and $\{\Pi_{A,1}\}$ are both sets of $2^{n-2}$ orthogonal projectors (by definition), and they all pairwise intersect (by assumption), the $\{\ket{\psi_A}\}$ will span a $2^{2n-4}$ dimensional space. Same with the $\{\ket{\psi_B}\}$.
    \item The $\{\ket{A}\}$ and the $\{\ket{B}\}$ are each contained in $\sX$, which is a $2^n$ dimensional space, and we know that \[\E_{(A,B) \in \cR}[\braket{A | B}] = 1/2.\]
    \item So, since the $\ket{\psi_A}$ are ``farther apart'' than the $\ket{A}$, and the $\ket{\psi_B}$ are ``farther apart'' than the $\ket{B}$, the expected inner product between $\ket{\psi_A}$ and $\ket{\psi_B}$ (for $(A,B) \gets \cR$) should be less than that of $\ket{A}$ and $\ket{B}$ (for $(A,B) \gets \cR$).
\end{itemize}



%\james{old below}
%First, define a symmetric binary relation $\cR$ on sets $\bS$ of $t$ sequences of $2n/3$-dimensional subspaces of $\bbF_2^n$, where $(\bS,\bT) \in \cR$ if for all $i \in [t]$, $S_i$ and $T_i$ overlap in exactly $2n/3 - 1$ dimensions. Then, we show that if there exists $U_\Com$ that violate \cref{claim:jor}, then \[\E_{\bS,\bT \gets \cR}[\braket{\psi_\bS|\psi_\bT}] \leq \frac{1}{2^{3t/2}}.\] However, since $\E_{\bS,\bT \gets \cR}[\braket{\bS|\bT}] = \frac{1}{2^t}$, the difference is nearly $\frac{1}{2^t}$, let's lower bound it by $\frac{1}{2^{t/2}}$. By small progress (Aaronson-Christiano), reducing the expectation by this much will take exponentially many queries in $n$, and if $n$ is set large enough compared to $t$, this contradicts the claim. Thus, it remains to bound the expectation above.

%To do this, we note that the following suffices. Fix any $\bS$ and state $\ket{\psi_\bS}$ that can depend arbitrarily on $\bS$. Then, we have that 

%\[\E_{\bT: (\bS,\bT) \in \cR}[\bra{\psi_\bS}\Jor[\bT]_\epsilon\ket{\psi_\bS}] \leq \frac{1}{\epsilon 2^{2t}} + \frac{1}{2^{\james{TBD}n}},\] where the expectation is over sampling a uniformly random $\bT$ such that $(\bS,\bT) \in \cR$.

%To analyze this, we imagine sampling $\bT$ in two steps: first $\bT_0$ and then $\bT_1$. That is, for each $i \in [t]$ we will sample $T_{i,0}$, and then for each $i \in [t]$ we will sample $T_{i,1}$. Note that $\mathsf{im}(\mathsf{Jor}[\bT]_\epsilon)$ is a subspace of $\mathsf{im}(\Pi[\bT^0])$. We will complete the analysis in three steps.

%\begin{enumerate}
    %\item Show that, for fixed $\bS$ and $\ket{\psi_\bS}$, \[\E_{\bT_0}[\bra{\psi_\bS}\Pi[\bT^0]\ket{\psi_\bS}] \leq \frac{1}{2^t} + \frac{1}{2^{\james{TBD}n}}.\]
    %\item Show that, for fixed $\bS,\bT_0$ and a state $\ket{\psi}$ defined based on $\bS,\bT_0$ (in fact, it will be in the image of $\Pi[\bT^0]$), \[\E_{\bT_1}[\bra{\psi}\Pi[\bT^1]\ket{\psi}] \leq \frac{1}{2^t}.\] This follows because given $\bS$ and $\bT_0$, there are exactly two choices for $\bT_1$, and they are disjoint from each other (except if $\bT_0 = \bS_0$ which is very unlikely, and anyway will then lead to a smaller expected overlap).
    %\item Note that, for any vector $\ket{\psi} \in \mathsf{im}(\Pi[\bT^0])$, it holds that \[\bra{\psi}\Pi[\bT^1]\ket{\psi} \geq \epsilon \cdot \bra{\psi}\mathsf{Jor}[\bT]_\epsilon\ket{\psi}.\]
%\end{enumerate}

\end{proof}


\iffalse
\subsection{Predicate binding}

Let $m = m(\secp)$ be any polynomial, and let $W_0,W_1 \in \{0,1,*\}^m$ be two sets such that for any $w_0 \in W_0$ and $w_1 \in W_1$, there exists $i \in [m]$ such that $w_{0,i},w_{1,i} \neq *$ and $w_{0,i} \neq w_{1,i}$. 

Let $\widehat{\bS} \coloneqq (\bS_1,\dots,\bS_M)$ be a sequence of $m$ sequences of subspace states $\bS_i$ and let $\ket{\widehat{\bS}}$ be the state $\ket{\bS_1}\dots\ket{\bS_m}$. Let $\SSC.\Gen^m(1^\secp,t,n)$ denote sampling $\SSC.\Gen(1^\secp,t,n)$ $m$ times. Let $O_{\widehat{\bS}}$ denote the sequence of oracles $O_{\bS_1},\dots,O_{\bS_m}$, and likewise for $O_{\widehat{\bS}}^\bot$. Finally, define \[\Pi_{\widehat{\bS}}^0 \coloneqq \sum_{w_0 \in W_0} \left(\bigotimes_{i: w_{0,i} \neq *}\Pi^{w_{0,i}}_{\bS_i} \right), \ \ \ \Pi_{\widehat{\bS}}^1 \coloneqq \sum_{w_1 \in W_1} \left(\bigotimes_{i: w_{1,i} \neq *}\Pi^{w_{1,i}}_{\bS_i} \right).\] Then we have the following corollary.


%Consider sampling $M$ sequences of subspaces $\widehat{S} \coloneqq (S^{(1)},\dots,S^{(M)})$, where each $S^{(i)}$ is sampled as above with parameters $t(\secp),n(\secp)$. 
%Define $O_{\widehat{S}}(k,i,v) \to \{\top,\bot\}$ to be an oracle that has hard-coded $\widehat{S} = (S^{(1)},\dots,S^{(N)})$ and outputs $O_{S^{(k)}}(i,v)$, and define $O_{\widehat{S}}^\bot(k,i,v) \to \{\top,\bot\}$ to be an oracle that has hard-coded $\widehat{S} = (S^{(1)},\dots,S^{(N)})$ and outputs $O_{S^{(k)}}^\bot(i,v)$



\begin{corollary}
For any polynomial $m = m(\secp)$, there exist polynomials $t = t(\secp)$ and $n = n(\secp)$ such that for any two-part adversary $(U_0,U_1)$, where $U_0$ and $U_1$ each make $\poly(\secp)$ many oracle queries, it holds that
\[\Pr_{\widehat{\bS} \gets \SSC.\Gen^m(1^\secp,t,n)}\left[\bra{\psi}\Pi_{\widehat{\bS}}^0\left({U_1^{O_{\widehat{\bS}}}}\right)^\dagger\Pi_{\widehat{\bS}}^1\left(U_1^{O_{\widehat{\bS}}}\right)\Pi_{\widehat{\bS}}^0\ket{\psi} \geq \frac{1}{\poly(\secp)} : \ket{\psi} \coloneqq U_0^{O_{\widehat{\bS}},O_{\widehat{\bS}}^\bot}(\ket{\widehat{\bS}})\right] = \negl(\secp).\]
\end{corollary}

\james{the overlap will go down by most $2^{2m}$ when we expand out the projectors. Then, we can set $p(\secp)$ and thus $t(\secp),n(\secp)$ appropriately }
\fi

==> obf-old.tex <==
\subsection{Construction}

In this section, we construct virtual black-box (VBB) obfuscation for pseudo-deterministic quantum circuits from the following ingredients.

\begin{itemize}
    \item A VBB obfuscator $(\CObf,\CEval)$ for classical circuits (\cref{def:ideal-obfuscation}).
    \item A quantum fully-homomorphic encryption scheme $(\QFHE.\Gen, \QFHE.\Enc, \QFHE.\Eval, \QFHE.\Dec)$ (\cref{subsec:QFHE}).
    \item A protocol for publicly-verifiable non-interactive classical verification of quantum partitioning circuits in the oracle model $(\PV.\Gen,\PV.\Prove,\PV.\Verify,\PV.\Out)$ (\cref{subsec:partitioning-def}).
\end{itemize}

The construction is given in \cref{fig:QObf}.

\protocol{Obfuscation scheme $(\QObf,\QEval)$ for pseudo-deterministic quantum circuits
}{Obfuscation for pseudo-deterministic quantum circuits.}{fig:QObf}{
\begin{itemize}
    \item $\QObf(1^\secp,Q)$:
    \begin{itemize}
        \item Sample $(\pk_\QFHE,\sk_\QFHE) \gets \QFHE.\Gen(1^\secp,D)$ and $\ct \gets \QFHE.\Enc(\pk_\QFHE,Q)$, where $D$ is the depth of $Q$.
        \item Let $E[\ct]$ be the circuit that takes $x$ as input and runs $\QFHE.\Eval(U[x],\ct)$, where $U[x]$ is the universal quantum circuit with $x$ hard-coded. That is, $U[x]$ takes as input the description of a quantum circuit $Q$ and outputs $Q(x)$.
        \item Sample $(\vk,\ket{\pk},\cPK) \gets \PV.\Gen(1^\secp,E[\ct])$.
        \item Let $\widetilde{\cPK} \gets \CObf(1^\secp,\cPK)$.
        \item Let $\cDK$ be the following functionality.
        \begin{itemize}
            \item Take $(x,\pi)$ as input.
            \item Compute $q \coloneqq \PV.\Ver(\vk,x,\pi)$ and output $\bot$ if $q = \bot$.
            \item Otherwise, output $b \coloneqq \PV.\Out(q,P[\sk_\QFHE])$, where $P[\sk_\QFHE](\cdot) \equiv \QFHE.\Dec(\sk_\QFHE,\cdot)$. 
        \end{itemize}
        \item Let $\widetilde{\cDK} \gets \CObf(1^\secp,\cDK)$.
        \item Output $\widetilde{Q} \coloneqq \left(\ct,\ket{\pk},\widetilde{\cPK},\widetilde{\cDK}\right)$.
    \end{itemize}
    \item $\QEval(\widetilde{Q},x)$:
    \begin{itemize}
        \item Parse $\widetilde{Q}$ as $\left(\ct,\ket{\pk},\widetilde{\cPK},\widetilde{\cDK}\right)$.
        \item Compute $\pi \gets \PV.\Prove^{\widetilde{\cPK}}(\ket{\pk},E[\ct],x)$.
        \item Output $b \coloneqq \widetilde{\cDK}(x,\pi)$.
    \end{itemize}
\end{itemize}

}

\begin{theorem}\label{thm:obfuscation}
$(\QObf,\QEval)$ described in \cref{fig:QObf} is a virtual black-box obfuscator for pseudo-deterministic quantum circuits, satisfying \cref{def:ideal-obfuscation}.
\end{theorem}

\begin{proof}
First, correctness follows immediately from the evaluation correctness of $\QFHE$ (\cref{def:eval correct}), and the completeness of $\PV$ (\cref{def:PV-completeness}). Note that even though the evaluation procedure may include measurements, an evaluator could run coherently, measure just the output bit $b$, and reverse. By Gentle Measurement (\cref{lemma:gentle-measurement}), this implies the ability to run the obfuscated program on any $\poly(\secp)$ number of inputs.

Next, we show security. For any QPT adversary $\{\sA_\secp\}_{\secp \in \bbN}$, we define a simulator $\{\sS_\secp\}_{\secp \in \bbN}$ as follows, where $\{\widetilde{\sA}_\secp\}_{\secp \in \bbN}$ is the simulator for the classical obfuscation scheme $(\CObf,\CEval)$, defined based on $\{\sA_\secp\}_{\secp \in \bbN}$.
\begin{itemize}
    \item Sample $(\pk_\QFHE,\sk_\QFHE) \gets \QFHE.\Gen(1^\secp,D)$, $\ct \gets \QFHE.\Enc(\pk_\QFHE,0^{|Q|})$, and $(\vk,\ket{\pk},\cPK) \gets \PV.\Gen(1^\secp,E[\ct])$.
    \item Run $\widetilde{\sA}_\secp^{\cPK,\cDK}(\ct,\ket{\pk})$, answering $\cPK$ calls honestly, and $\cDK$ calls as follows. 
    \begin{itemize}
        \item Take $(x,\pi)$ as input.
        \item Compute $q \coloneqq \PV.\Ver(\vk,x,\pi)$ and output $\bot$ if $q = \bot$.
        \item Otherwise, forward $x$ to the external oracle $O[Q]$, and return the result $b = O[Q](x)$.
    \end{itemize}
    \item Output $\widetilde{\sA}_\secp$'s output.
\end{itemize}

Now, for any circuit $Q$, we define a sequence of hybrids.

\begin{itemize}
    \item $\cH_0$: Sample $\widetilde{Q} \gets \QObf(1^\secp,Q)$ and run $\sA_\secp(1^\secp,\widetilde{Q})$.
    \item $\cH_1$: Sample $(\ct,\ket{\pk},\cPK,\cDK)$ as in $\QObf(1^\secp,Q)$, and run $\widetilde{\sA}_\secp^{\cPK,\cDK}(\ct,\ket{\pk})$.
    \item $\cH_2$: Same as $\cH_1$, except that calls to $\cDK$ are answered as in the description of $\sS_\secp$.
    \item $\cH_3$: Same as $\cH_2$, except that $\ct$ is sampled as $\ct \gets \QFHE.\Enc(\pk_\QFHE,0^{|Q|})$. This is $\sS_\secp$.
\end{itemize}

We complete the proof by showing the following.

\begin{itemize}
    \item $|\Pr[\cH_0 = 1] - \Pr[\cH_1 = 1]| = \negl(\secp)$. This follows from the security of the classical obfuscation scheme $(\CObf,\CEval)$.
    \item $|\Pr[\cH_1 = 1] - \Pr[\cH_2 = 1]| = \negl(\secp)$. Suppose otherwise. Then there must exist some query made by $\widetilde{\sA}_\secp$ to $\cDK$ with noticeable amplitude on $(x,\pi)$ such that $q \neq \bot$ and $\PV.\Out(q,P[\sk_\QFHE]) = 1-Q(x)$, where $q = \PV.\Ver(\vk,x,\pi)$. Thus, we can measure a random one of the $\poly(\secp)$ many queries made by $\widetilde{\sA}_\secp$ to obtain such an $(x,\pi)$ with noticeable probability. However, since $P[\sk_\QFHE] \circ E[\ct] \equiv Q$ is pseudo-deterministic, this violates the soundness of $\PV$ (\cref{def:PV-soundness}).
    \item $|\Pr[\cH_2 = 1] - \Pr[\cH_3 = 1]| = \negl(\secp)$. Since $\sk_\QFHE$ is no longer used in $\cH_2$ to respond to $\cDK$ queries, this follows from the semantic security of $\QFHE$ (\cref{def:semantic-security}).
\end{itemize}

\end{proof}
